Cognitive Noise and Altruistic Preferences

I study altruistic choices through the lens of a cognitively noisy decision-maker. I introduce a theoretical framework that demonstrates how increased cognitive noise can directionally affect altruistic decisions and put its implications to the test: In a laboratory experiment, participants make a series of binary choices between taking and giving monetary payments. In the treatment, to-be-calculated math sums replace straightforward monetary payments, increasing the cognitive difficulty of choosing. The Treatment group exhibits a lower sensitivity towards changes in payments and decides significantly more often in favor of the other person, i.e., is more altruistic. I explore the origins of this effect with Bayesian hierarchical models and a number-comparison task, mirroring the "mechanics" of the altruism choices absent any altruistic preference. The treatment effect is similar in this task, suggesting that the perception of numerical magnitudes drives treatment differences. The probabilistic model supports this interpretation. A series of additional results show a negative correlation between cognitive reflection and individual measures of cognitive noise, as well as associations between altruistic choice and number comparison. Overall, these results suggest that the expression of altruistic preferences -- and potentially social preferences more generally -- is affected by the cognitive difficulty of their implementation.

==> 0_0_Preamble/Preamble_BibLaTeX_AER.tex <==
% !TeX program = pdflatex
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !BIB program = biber
% !TeX TXS-program:bibliography = txs:///biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  CITATION COMMANDS AND BIBLIOGRAPHY STYLE  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% AER/JEL/JEP style

\usepackage[
	authordate, backend = biber, natbib = true, doi = only, isbn = false,
	sorting = ynt, sortcites = true,  % sort the in-text citations by year of publication
	compresspages = true, dashed = false,
	backref = true, backrefstyle = three,
	bibencoding = inputenc, citetracker = true
]{biblatex-chicago}

\urlstyle{same}  % Since biblatex-chicago sets \urlstyle{rm}
% See https://tex.stackexchange.com/questions/134191/line-breaks-of-long-urls-in-biblatex-bibliography:
\setcounter{biburllcpenalty}{10000}
\setcounter{biburlucpenalty}{10000}
\setcounter{biburlnumpenalty}{10000}
\AtBeginDocument{\biburlbigskip = 0mu\relax}  % To prevent excessive whitespace in URLs and DOIs

\DeclareDelimFormat{nameyeardelim}{\addcomma\space}
\let \citeorig \cite
\renewcommand{\cite}{\citet}
\renewcommand{\citealp}{\citeorig}
\AtBeginDocument{\setlength{\bibhang}{\baselineskip}}
\DeclareFieldFormat[report]{title}{\mkbibquote{#1}}
\AtBeginDocument{%
	\iftoggle{cms@comprange}
		{\DeclareFieldFormat{pages}{\addspace\mbox{\mkcomprange{#1}}}}%
		{\DeclareFieldFormat{pages}{\addspace\mbox{\mknormrange{#1}}}}%
}%
% Make author/editor name(s) bold
\xpatchbibmacro{author}{\usebibmacro{justauthor}}{\mkbibbold{\usebibmacro{justauthor}}}{}{}
\xpatchbibmacro{author}{\usebibmacro{moreauthor}}{\mkbibbold{\usebibmacro{moreauthor}}}{}{}

%\usepackage[backend=biber, natbib=true, bibencoding=inputenc, bibstyle=authoryear, citestyle=authoryear-comp, mincitenames=1, maxcitenames=3, minbibnames=99, maxbibnames=99, uniquename=false, uniquelist=true, backref=true, backrefstyle=three, doi=true, isbn=false, dashed=false, sorting=ynt, sortcites=true, mergedate=true, dateabbrev=false, abbreviate=false, citetracker=true]{biblatex}
% sortcites sorts the in-text citations by year of publication
\DeclareBibliographyAlias{newspaper}{article}

\defbibheading{subbibliography}[\refname]{%
	\section*{#1}%
	\sectionmark{#1}%
	\addcontentsline{toc}{section}{#1}%
}

\renewcommand{\bibfont}{\sffamily\small}
	% Reduce font size for the bibliography, make the font sans-serif.
\setlength{\bibindent}{\parindent}
\setlength{\bibitemsep}{0pt}

\DefineBibliographyStrings{english}{%
	andothers = {et~al\adddot},
	volume = {vol\adddot}
}

% Handling of newspaper articles
\DeclareFieldFormat[newspaper]{journaltitle}{%
	\mkbibemph{#1} \mkbibparens{\thefield{edition}}\addcomma\addspace%
	\iflanguage{ngerman}{%
		\addnbspace\thefield{day}\addperiod\addnbspace\mkbibmonth{\thefield{month}}\addspace\thefield{year}%
	}{% else: default to the USenglish version
		\mkbibmonth{\thefield{month}}\addnbspace\thefield{day}\addcomma\addspace\thefield{year}%
	}%
	\iffieldundef{volume}{\addcolon}{\addcomma}%
}
\DeclareFieldFormat[newspaper]{date}{%
	\thefield{year}%
}

% Adjust formatting of back-references
% ==>
\DefineBibliographyStrings{english}{%
	backrefpage  = {},	% originally ``cit. on p.''
	backrefpages = {}	% originally ``cit. on pp.''
}
\DefineBibliographyStrings{ngerman}{%
	backrefpage  = {},	% originally ``Siehe Seite''
	backrefpages = {}	% originally ``Siehe Seiten''
}
\renewcommand*{\finentrypunct}{}
\renewbibmacro*{pageref}{%
	\addperiod
	\iflistundef{pageref}
	{}
	{\printtext[brackets]{%
			\ifnumgreater{\value{pageref}}{1}
				{\bibstring{backrefpages}}
				{\bibstring{backrefpage}}%
			\printlist[pageref][-\value{listtotal}]{pageref}%
		}%
	}%
}
% <==

% Move notes to the end of an entry by copying the ``note'' information into ``addendum'': -->
\DeclareSourcemap{
	\maps[datatype=bibtex]{
		% Copy values of the Mendeley-created ``annote'' field to the ``note'' field:
		\map[overwrite]{
		 	\step[fieldsource=annote]
		 	\step[fieldset=note, origfieldval, append]
			\step[fieldset=annote, null]
		}
		\map{
			\step[fieldsource=note, final]
			\step[fieldset=addendum, origfieldval, final]
			\step[fieldset=note, null]
		}
	}
}
% \DeclareFieldFormat{addendum}{(#1)} % Enclose addendum/note in parentheses.
% <--

\AtEveryBibitem{%
	\ifentrytype{newspaper}%
		{\clearfield{addendum}}% then
		{\clearfield{month}}% else
}

% Add ``working paper'' as the default value for type of ``techreports'' ==>
% see https://tex.stackexchange.com/questions/212362/how-to-use-declaresourcemap-to-add-default-value-to-a-field
\DeclareSourcemap{
	\maps[datatype=bibtex]{
		\map{% Will overwrite fields without the ``overwrite'' option
			\pertype{techreport}
			\step[fieldset=type, fieldvalue={Working paper}]
		}
	}
}
% <==

% Add “doctoral dissertation” as the default value for type of “phdthesis” ==>
% see https://tex.stackexchange.com/questions/212362/how-to-use-declaresourcemap-to-add-default-value-to-a-field
\DeclareSourcemap{
	\maps[datatype=bibtex]{
		\map{% Will overwrite fields without the ``overwrite'' option
			\pertype{phdthesis}
			\step[fieldset=type, fieldvalue={Doctoral dissertation}]
		}
	}
}
% <==

% Remove superfluous ``The'' from journal names ==>
\DeclareSourcemap{
	\maps[datatype=bibtex]{
		\map{
			\step[fieldsource=journal, match={\regexp{^The\s}}, replace={}]
		}
	}
}
% <==

% Replace (Mendeley's) month strings (``jan'', ``feb'', etc.) by full names ==>
\DeclareSourcemap{
	\maps[datatype=bibtex]{
		\map{
			\step[fieldsource=number, match={\regexp{^jan$}}, replace=\regexp{\\mkbibmonth\{1\}}]
			\step[fieldsource=number, match={\regexp{^feb$}}, replace=\regexp{\\mkbibmonth\{2\}}]
			\step[fieldsource=number, match={\regexp{^mar$}}, replace=\regexp{\\mkbibmonth\{3\}}]
			\step[fieldsource=number, match={\regexp{^apr$}}, replace=\regexp{\\mkbibmonth\{4\}}]
			\step[fieldsource=number, match={\regexp{^may$}}, replace=\regexp{\\mkbibmonth\{5\}}]
			\step[fieldsource=number, match={\regexp{^jun$}}, replace=\regexp{\\mkbibmonth\{6\}}]
			\step[fieldsource=number, match={\regexp{^jul$}}, replace=\regexp{\\mkbibmonth\{7\}}]
			\step[fieldsource=number, match={\regexp{^aug$}}, replace=\regexp{\\mkbibmonth\{8\}}]
			\step[fieldsource=number, match={\regexp{^sep$}}, replace=\regexp{\\mkbibmonth\{9\}}]
			\step[fieldsource=number, match={\regexp{^oct$}}, replace=\regexp{\\mkbibmonth\{10\}}]
			\step[fieldsource=number, match={\regexp{^nov$}}, replace=\regexp{\\mkbibmonth\{11\}}]
			\step[fieldsource=number, match={\regexp{^dec$}}, replace=\regexp{\\mkbibmonth\{12\}}]
		}
	}
}
% <==

==> 0_0_Preamble/Preamble_Fonts_IBMPlex.tex <==
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !TeX TXS-program:bibliography = txs:///biber
% !BIB program = biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FONT SETTINGS AND TYPOGRAPHY  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Use Fira Sans as the sans-serif font.
% Load first because it otherwise doesn't work properly.
% ==>
%\usepackage[lining, scale=0.88]{FiraMono}  % To match the x-height of the Charter serif font
%\usepackage[book, semibold, lining, tabular, scale=0.88]{FiraSans}[2018/05/23]
%\makeatletter
%\@ifpackagelater{FiraSans}{2018/05/23}
%	{}
%	{\PackageError{FiraSans}
%	     {Outdated 'FiraSans' package}
%	     {Upgrade to FiraSans 2018/05/23 or newer!\MessageBreak
%	      Otherwise the sans-serif font may not work properly, or the compilation might fail.\MessageBreak
%	      This is a fatal error. I'm aborting now.}%
%	\endinput%
%   }
%\makeatother
%% In case you wish to use the ``light'' options of FiraSans: -->
%\ifthenelse{\isundefined{\AfterPackage}}{\usepackage{afterpackage}}{}
%\AfterPackage{siunitx}{%
%  \providecommand*{\lseries}{\fontseries{l}\selectfont}
%}
% See https://tex.stackexchange.com/questions/164791/combination-of-siunitx-and-light-weight-font-fails-to-compile.
% <--
% <==

\usepackage[xcharter, slantedGreek, scaled=1.055, upint]{newtxmath}
%\usepackage[xcharter, slantedGreek, scaled=1.09]{newtxmath}
% This template also works with the ``IBM Plex Sans'' and ``IBM Plex Mono'' fonts,
% https://ctan.org/pkg/plex ==>
\usepackage[textmd, semibold, scale=0.91]{plex-mono}  % To match the x-height of the Charter serif font
\usepackage[textmd, semibold, scale=0.91]{plex-sans}[2018/12/31]
% Earlier versions of the ``plex-sans'' package do not include support for LGR Greek.
% <==

%% This template also works with the ``Alegreya'' and ``Alegreya Sans'' fonts,
%% https://ctan.org/pkg/alegreya ==>
%\usepackage[semibold, scale=0.89]{plex-mono}  % To match the x-height of the Charter serif font
%\usepackage[lining, tabular, scale=1.02]{AlegreyaSans}[2018/08/02]
%	% Earlier versions of the ``Alegreya'' package do not include support for LGR Greek.
%% <==

%% This template also works with the ``Google Noto'' fonts,
%% https://ctan.org/pkg/noto ==>
%\usepackage[scale=0.85]{noto-mono}
%\usepackage[lining, tabular, scale=0.85]{noto-sans}[2019/01/11]
%	% Earlier versions of the ``noto'' package do not include support for LGR Greek.
%% <==

% Save the font family and font series definitions for later use: ==>
\newcommand{\savesffamily}{\sfdefault}
\makeatletter
\newcommand{\savesfmdseries}{\mdseries@sf}
\newcommand{\savesfbfseries}{\bfseries@sf}
\makeatother
% <==

% Use Bitstream Charter as the math font
% ==>
%\usepackage[charter, greeklowercase=italicized, greekuppercase=italicized, sfscaled=false, ttscaled=false]{mathdesign}
%% Use Alegreya as the text font -->
%\usepackage[lining, tabular, scale=1.02]{Alegreya}[2018/08/02]
%\ifxetex \else \DisableLigatures[T]{family = {rm*}} \fi
%% <--
%% Use Noto Serif as the text font -->
%\usepackage[lining, tabular, scale=0.85]{noto-serif}[2019/01/11]
%% <--
% Use IBM Plex as the text font -->
\usepackage[textmd, semibold, scale=0.91]{plex-serif}
% <--
% Save the font family and font series definitions for later use:
\let \savermfamily \rmdefault
\makeatletter
\newcommand{\savermmdseries}{\mdseries@rm}
\newcommand{\savermbfseries}{\bfseries@rm}
\makeatother
% <==

% mathdesign provides upright Greek letters as \alphaup, \Betaup, etc. while other packages
% (e.g., unicode-math) call these \upalpha, \upBeta, etc. We make also the latter available.
% ==>
\makeatletter
\@for\@tempa:=%
	alpha,beta,gamma,delta,epsilon,varepsilon,zeta,eta,theta,vartheta,iota,kappa,lambda,mu,nu,xi,%
	omicron,pi,varpi,rho,varrho,sigma,varsigma,tau,upsilon,phi,varphi,chi,psi,omega,digamma,%
	Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
	Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
\do{%
	\expandafter\let\csname up\@tempa\expandafter\endcsname\csname\@tempa up\endcsname%
}%
\makeatother
% <==

% Provide a \nequiv symbol
\ifx\nequiv\undefined
	\newcommand{\nequiv}{\not\equiv}
\fi

% Use Bitstream Charter as the text font
% ==>
%\usepackage[scaled=.96, lining, sups]{XCharter}  % option ``sups'' not working properly with subimport
% Save the font family and font series definitions for later use:
\let \savermdefaultfortext \rmdefault
\let \savemddefaultfortext \mddefault
\let \savebfdefaultfortext \bfdefault
\renewcommand{\textellipsis}{\mbox{.{\kern.09em}.{\kern.09em}.}}
%\makeatletter
%\newcommand{\@makefnmarkorig}{%
%	\hbox{\sufigures\hspace*{.04em}\@thefnmark\hspace*{.04em}}%
%}  % Copied from XCharter.sty
%\makeatother
% <==

\ifxetex
	% Do nothing.
\else
	\DisableLigatures[f]{family = {rm*, sf*, tt*}}
	% Disable the f* ligatures for the Plex fonts because the fonts do not provide sufficient support.
	% Disable the f* ligatures for the ``typewriter'' font because they make no sense for a monospaced font.
	\SetExtraKerning[unit=space]
		{encoding=*, family=*, series=*, size={*, normalsize, footnotesize}, font = */*/*/*/*}
		{\textemdash = {325, 325},
			/ = {100, 100},
			: = { 50,   0},
			; = { 50,   0}}
\fi

\usepackage{xfrac}	% Provides \sfrac

% Since math mode uses a different font encoding, issuing \euro/\texteuro in math mode
% produces an incorrect sign. We fix this. ==>
\AtBeginDocument{%
	\providecommand{\euro}[1]{%
		\relax\ifmmode\text{\texteuro}#1\else\texteuro #1\fi%
	}%
}
% <==

==> 0_0_Preamble/Preamble_Fonts_Times.tex <==
% !TeX program = pdflatex
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !BIB program = biber
% !TeX TXS-program:bibliography = txs:///biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FONT SETTINGS THESIS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{amsfonts, amssymb}  % Additional symbols from AMS
%\usepackage{amsfonts}  % Additional symbols from AMS
\usepackage{extarrows}

% Use Times Roman for text and math
%\usepackage{newtxtext}
%\usepackage[smallerops, varg, upint, slantedGreek]{newtxmath}

%\usepackage[scale=1.07]{tgcursor}
%	% Use Courier as the typewriter font
%\usepackage[scale=0.93]{sourcecodepro}
%	% Use Source Code Pro as the typewriter font
\usepackage[scaled=0.835]{DejaVuSansMono}  % Scaled to match the x-height of the newtxtext Times Roman
	% Use DejaVu Sans Mono as the typewriter font, also supports Greek via the LGR encoding

\usepackage{xfrac}

\usepackage[protrusion=true, expansion=false, kerning=true]{microtype}
% This package enables so-called hanging punctuation. That is, when a punctuation sign like ":", ".", "-", etc. is found at the beginning or end of a line, it is protruded a little into the page margin. This results in "optical margin alignment," because the protrusion makes the margin alignment look straighter.
%\DisableLigatures[f]{family = {sf*, rm*}}
%	% Disable the f* ligatures for both Fira Sans and Charter because both fonts provide insufficient support
%\DisableLigatures[f]{family = {rm*}}
	% Disable the f* ligatures for Charter because it provides insufficient support
\SetExtraKerning[unit=space]
{encoding=*, family=*, series=*, size={*, normalsize, footnotesize}, font = */*/*/*/*}
{\textemdash = {325, 325},
	/ = {100, 100},
	: = { 50,   0},
	; = { 50,   0}}
\renewcommand{\textellipsis}{\mbox{.{\kern.09em}.{\kern.09em}.}}

\renewcommand{\bibfont}{%
	\normalsize%
	\addtolength{\baselineskip}{0.05\baselineskip}%
	%\setlength{\baselineskip}{\newbaselineskip}%
}  % Use same size for bibliography as for body text.

\captionsetup{footfont={rm, footnotesize}}  % Set font in \floatfoot to serif and footnotesize




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  MATH-RELATED ADJUSTMENTS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{mathrsfs}  % Provides the \mathscr math alphabet

% The following is taken from
% https://tex.stackexchange.com/questions/116389/automatic-upright-math-when-text-is-in-italic/116399#116399
% Filling in ``missing'' Greek glyphs for completeness
% (not really necessary, since they look identical to Latin glyphs and are thus almost never used)
% ==>
\newcommand{\omicron}{o}
\newcommand{\Digamma}{F}
\newcommand{\Alpha}  {A}
\newcommand{\Beta}   {B}
\newcommand{\Epsilon}{E}
\newcommand{\Zeta}   {Z}
\newcommand{\Eta}    {H}
\newcommand{\Iota}   {I}
\newcommand{\Kappa}  {K}
\newcommand{\Mu}     {M}
\newcommand{\Nu}     {N}
\newcommand{\Omicron}{O}
\newcommand{\Rho}    {P}
\newcommand{\Tau}    {T}
\newcommand{\Chi}    {X}
% <==

% Upright Greek letters for the \mathup command
% ==>
\makeatletter
% Save original definitions of the Greek letters
\@for\@tempa:=%
	alpha,beta,gamma,delta,epsilon,varepsilon,zeta,eta,theta,vartheta,iota,kappa,lambda,mu,nu,xi,%
	omicron,pi,varpi,rho,varrho,sigma,varsigma,tau,upsilon,phi,varphi,chi,psi,omega,digamma,%
	Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
	Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
\do{%
	\expandafter\let\csname\@tempa orig\expandafter\endcsname\csname\@tempa\endcsname%
	\expandafter\let\csname\@tempa uporig\expandafter\endcsname\csname\@tempa up\endcsname%
}%
\newcommand*{\upgreekletters}{%
	\@for\@tempa:=%
		alpha,beta,gamma,delta,epsilon,varepsilon,zeta,eta,theta,vartheta,iota,kappa,lambda,mu,nu,xi,%
		omicron,pi,varpi,rho,varrho,sigma,varsigma,tau,upsilon,phi,varphi,chi,psi,omega,digamma,%
		Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
		Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa up\endcsname%
	}%
}
\newcommand*{\itgreekletters}{%
	\@for\@tempa:=%
		alpha,beta,gamma,delta,epsilon,varepsilon,zeta,eta,theta,vartheta,iota,kappa,lambda,mu,nu,xi,%
		omicron,pi,varpi,rho,varrho,sigma,varsigma,tau,upsilon,phi,varphi,chi,psi,omega,digamma,%
		Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
		Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa orig\endcsname%
	}%
}
\makeatother
% <==

\newcommand{\mathup}[1]{\upgreekletters\mathrm{#1}\itgreekletters}

\renewcommand{\mathbf}[1]{\bm{#1}}
\newcommand{\mathbfit}[1]{\mathbf{\mathit{#1}}}
\newcommand{\mathbfup}[1]{\upgreekletters\mathbf{\mathrm{#1}}\itgreekletters}

% Since math mode uses a different font encoding, issuing \euro/\texteuro in math mode
% produces an incorrect sign. We fix this. ==>
\AtBeginDocument{%
	\newcommand*{\euro}[1]{%
		\relax\ifmmode\text{\texteuro}#1\else\texteuro #1\fi%
	}%
}
% <==

==> 0_0_Preamble/Preamble_Page_layout_dissertation.tex <==
% !TeX program = pdflatex
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !BIB program = biber
% !TeX TXS-program:bibliography = txs:///biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  PAGE LAYOUT: ADDITIONAL SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Increase text width and text height by 5% to make the text
% flow exactly as in \documentclass[a4paper, 10pt]{article}
% ==>
%\addtolength{\textheight}{0.05\textheight}
%\addtolength{\textwidth}{0.05\textwidth}
%\addtolength{\evensidemargin}{-0.05\textwidth}
% <==

\usepackage[sf, bf, raggedright, explicit]{titlesec}	% Sansserif font for the headings
% Page headers
% ==>
\addtolength{\topmargin}{-14.25pt}
\addtolength{\headsep}{14.25pt}
	% Move header up so that the distance to the body text increases;
	% it should be approximately as large as the largest space above a heading.
\newpagestyle{chapterleftsectionright}[\small\sffamily\selectfont]{
	\sethead%
	[\textbf{\thepage}~~|~~%
	 \ifthechapter{\thechapter~~}{}\ecapitalisewords{\chaptertitle}%
	 \strut%
	]% even-left
	[]% even-center
	[]% even-right
	{}% odd-left
	{}% odd-center
	{\ifx\sectiontitle\empty%
		\ifthechapter{\thechapter~~}{}\ecapitalisewords{\chaptertitle}%
	 \else%
		\ifthesection{\thesection~~}{}\ecapitalisewords{\sectiontitle}%
	 \fi%
	 ~~|~~\textbf{\thepage}%
	 \strut%
	}%	odd-right
}
\newpagestyle{chapterleftappendixsectionright}[\small\sffamily\selectfont]{
	\sethead%
	[\textbf{\thepage}~~|~~%
	 \ifthechapter{\thechapter~~}{}\ecapitalisewords{\chaptertitle}%
	 \strut%
	]% even-left
	[]% even-center
	[]% even-right
	{}% odd-left
	{}% odd-center
	{\ifx\sectiontitle\empty%
		\ifthechapter{\thechapter~~}{}\ecapitalisewords{\chaptertitle}%
	 \else%
		\appendixname~\ifthesection{\thesection~~}{}\ecapitalisewords{\sectiontitle}%
	 \fi%
	 ~~|~~\textbf{\thepage}%
	 \strut%
	}%	odd-right
}
\pagestyle{chapterleftsectionright}
\definecolor{almostwhite}{RGB}{254,254,254}
% Some printers skip completely empty pages. To avoid this, we put a tiny gray period in ``empty'' headers:
\renewpagestyle{empty}[\tiny\selectfont]{
	\sethead%
	[]% even-left
	[]% even-center
	[\textcolor{almostwhite}{.}]% even-right
	{\textcolor{almostwhite}{.}}% odd-left
	{}% odd-center
	{}% odd-right
}
\usepackage{emptypage}  % Suppresses page numbers and headings from appearing on empty pages.
\assignpagestyle{\chapter}{empty} % Make footer empty on starting page of a new chapter
% <==

% Remove indent from the list of figures and list of tables
% ==>
%\usepackage{titletoc}
%\newcommand{\tocdots}{\titlerule*{\hspace{.8pc}.\hspace{-.45pc}}}
%\contentsmargin{2.55em}
%\titlecontents{chapter}
%	[1.5em]
%	{\addvspace{1ex}}
%	{\large\sffamily\bfseries\contentslabel{1.5em}}{\hspace*{-1.5em}\large\sffamily\bfseries}  % The latter ``outdents'' unnumbered sections; large wbold and sans-serif chapter entries in ToC
%	{\large\sffamily\bfseries\titlerule*{}\contentspage[\thecontentspage\hspace{-.12em}]}
%\titlecontents{section}
%	[3.8em] % = 1.5em + 2.3em, 1.5em reserved for chapter numbering
%	{\addvspace{0.25ex}}
%	{\bfseries\contentslabel{2.3em}}{\hspace*{-2.3em}}  % The latter ``outdents'' unnumbered sections, bold section entries in ToC
%	{\titlerule*{}\contentspage}%{\tocdots\contentspage}
%\titlecontents{subsection}
%	[6.8em] % = 1.5em + 2.3em + 3em, 1.5em + 2.3em reserved for chapter and section numbering
%	{}{\contentslabel{3em}}{\hspace*{-3em}}  % The latter ``outdents'' unnumbered subsections
%	{\titlerule*{}\contentspage}%{\tocdots\contentspage}
%\newlength{\loflotleft} \setlength{\loflotleft}{3.5em}
%\titlecontents{figure}
%	[\loflotleft]
%	{}{\contentslabel{\loflotleft}}{}
%	{\titlerule*{}\contentspage}%{\tocdots\contentspage}
%\titlecontents{table}
%	[\loflotleft]
%	{}{\contentslabel{\loflotleft}}{}
%	{\titlerule*{}\contentspage}%{\tocdots\contentspage}
% <==

%% Remove the leader (dots) from the table of contents, see
%% https://tex.stackexchange.com/questions/73789/how-to-remove-the-dots-in-the-tableof-contents
%% ==>
%\makeatletter
%\renewcommand{\@dotsep}{10000} 
%\makeatother
%% <==

\usepackage[titles]{tocloft}
\renewcommand{\cftdotsep}{\cftnodots}  % Remove the leader (dots) from the table of contents
\renewcommand{\cftchapfont}{\large\sffamily\bfseries}
\renewcommand{\cftchappagefont}{\cftchapfont}
\apptocmd{\cftchapfillnum}{\nopagebreak}{}{}  % Prevent page breaks after chapter entry in table of contents
%\renewcommand{\cftsecfont}{\bfseries}  % Make section entries in the table of contents bold
%\renewcommand{\cftsecpagefont}{\cftsecfont}
\setlength{\cftbeforesecskip}{\smallskipamount-0.1em}
\setlength{\cftfigindent}{0pt}  % Remove indentation from list of figures
\setlength{\cfttabindent}{0pt}  % Remove indentation from list of tables
\setlength{\cftfignumwidth}{3.75em}  % Make labels in LoF wider
\setlength{\cfttabnumwidth}{3.75em}  % Make labels in LoT wider
\setlength{\cftbeforesubsecskip}{-0.05em}
% Prevent unwanted optical marginal alignment of page numbers by microtype:
\newlength{\cftaux}
\renewcommand{\cftfigafterpnum}{\phantom{\,}\settowidth{\cftaux}{\,}\hspace{-\cftaux}}
\renewcommand{\cfttabafterpnum}{\phantom{\,}\settowidth{\cftaux}{\,}\hspace{-\cftaux}}


%%%% ALEX CHANGE TOC Spacing between cahpters

\makeatletter
\newskip\old@cftbeforechapskip
\old@cftbeforechapskip\cftbeforechapskip
\let\old@l@chapter\l@chapter
\let\old@l@section\l@section
\def\l@chapter#1#2{\old@l@chapter{#1}{#2}\cftbeforechapskip5pt}% set your value here
\def\l@section#1#2{\old@l@section{#1}{#2}\cftbeforechapskip\old@cftbeforechapskip}
\makeatother

%%ALEX ADDITIONAL
%\cftsetrmarg{5em}
\makeatletter
\renewcommand{\@tocrmarg}{4em}
\makeatother

\setcounter{secnumdepth}{3}
	% So that also 3rd-level headings are numbered.
	% Note: chapter is level 0, hence \subsubsection is actually on the 4th level.

\newcommand{\TestForPunct}[1]{\iftextterm{#1}{#1}{#1\unskip.}}
	% Adds a period if no punctuation mark is present yet

\titleformat{\chapter}[display]
	{\sffamily\fontseries{medium}\huge}%\sffamily\bfseries\addfontfeature{Numbers=Lining}
	{\scalefont{0.95}\chaptertitlename~\thechapter}% {\thechapter}
	{1.5\bigskipamount}%
	{\sffamily\fontseries{l}\linespread{0.95}\Huge\raggedright%
	 \xcapitalisewords{%
		#1%
	 }%
	}

%\newlength{\appendixlabellength}
\newcommand{\appendixformat}[1][\currentname]{%
	\pagestyle{chapterleftappendixsectionright}%
	\titleformat{\section}[hang]
		{\raggedright\Large\sffamily\bfseries}{\appendixname~\thesection\quad}{0pt}{%
			\ecapitalisewords{%
				#1%
			}%
		}[]%
%	\setlength{\appendixlabellength}{\widthof{\textbf{\appendixname~}}+2.3em}%
%	\titlecontents{section}
%		[\appendixlabellength+1.5em] % = 1.5em + 2.3em, 1.5em reserved for chapter numbering
%		{\addvspace{0.25ex}}
%		{\bfseries\contentslabel[\appendixname~\thecontentslabel]{\appendixlabellength}}{}
%		{\titlerule*{}\contentspage}%{\tocdots\contentspage}
}
\AtBeginEnvironment{appendix}{\appendixformat}
\AtBeginEnvironment{appendices}{\appendixformat}
\AtBeginEnvironment{subappendices}{\appendixformat}
\AtEndEnvironment{appendix}{%
%	\pagestyle{chapterleftsectionright}%
	\thispagestyle{chapterleftappendixsectionright}%
}
\AtEndEnvironment{appendices}{%
%	\pagestyle{chapterleftsectionright}%
	\thispagestyle{chapterleftappendixsectionright}%
}
\AtEndEnvironment{subappendices}{%
%	\pagestyle{chapterleftsectionright}%
	\thispagestyle{chapterleftappendixsectionright}%
}

\titleformat{name=\section}[hang]
	{\raggedright\Large\sffamily\bfseries}{\thesection\quad}{0pt}{%
		\xcapitalisewords{%
			#1%
		}%
	}[]
\titleformat{name=\section, numberless}[hang]
	{\raggedright\Large\sffamily\bfseries}{}{0pt}{%
		\xcapitalisewords{%
			#1%
		}%
	}[]
\titleformat{name=\subsection}[hang]
	{\raggedright\large\sffamily\bfseries}{\thesubsection\quad}{0pt}{%
		\xcapitalisewords{%
			#1%
		}%
	}[]
\titleformat{name=\subsection, numberless}[hang]
	{\raggedright\large\sffamily\bfseries}{}{0pt}{%
		\xcapitalisewords{%
			#1%
		}%
	}[]
\titleformat{name=\subsubsection}[hang]
	{\raggedright\large\sffamily\bfseries}{\thesubsubsection\quad}{0pt}{%
		\xcapitalisewords{%
			#1%
		}%
	}[]
\titleformat{name=\subsubsection, numberless}[hang]
	{\raggedright\large\sffamily\bfseries}{}{0pt}{%
		\xcapitalisewords{%
			#1%
		}%
	}[]
\titleformat{name=\paragraph, numberless}[runin]
	{}{}{0pt}{%
		\textbf{%
			#1\iftextterm{#1}{}{\unskip}%
		}%
	}[]
\titleformat{name=\subparagraph, numberless}[runin]
	{}{}{0pt}{%
		\textbf{%
			#1\iftextterm{#1}{}{\unskip.}%
		}%
	}[]
\titlespacing{\paragraph}
	{0pt}{0.5\baselineskip plus 0.5\baselineskip}{3\wordsep}[]
\titlespacing{\subparagraph}
	{\parindent}{0pt}{3\wordsep}[]

\AtBeginDocument{%
	\captionsetup{footfont={sf, footnotesize}}
		% Set font in \floatfoot to sans-serif and footnotesize
}

% \marginpar settings for the commenting functions
%\setlength{\marginparwidth}{3.75cm}
%\setlength{\marginparsep}{0.4cm}
%\setlength{\marginparpush}{0.4cm}

==> 0_0_Preamble/Preamble_Sansserif_math_IBMPlex.tex <==
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX program = pdflatex




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  SANS-SERIF MATH IN SANS-SERIF ENVIRONMENT  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% See https://tex.stackexchange.com/questions/41497/how-to-typeset-some-text-including-math-content-in-sans-serif
% See https://tex.stackexchange.com/questions/33165/make-mathfont-respect-the-surrounding-family

% Necessary for use of kpfonts
% ==>
\makeatletter
\newif\ifkp@upRm
\newif\ifkp@osm
\newif\ifkp@vosm
\makeatother
% <==

\DeclareMathVersion{normalup}
\DeclareMathVersion{boldup}
\DeclareMathVersion{sans}

%\DeclareSymbolFont{operators}{OT1}{ntxtlf}{m}{n}

%\SetSymbolFont{operators}{normal}{OT1}{ntxtlf}{m}{n}
%\SetSymbolFont{operators}{bold}  {OT1}{ntxtlf}{bx}{n}

%\SetSymbolFont{operators}{sans}{OT1}{jkpss}{m}{n}
%	% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{operators}   {sans}{OT1}{ntxtlf}{m}{n}
%\SetSymbolFont{letters}     {sans}{OML}{jkpss}{m}{it}
% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{letters}     {sans}{OML}{cmbrm}{m}{it}
%\SetSymbolFont{symbols}     {sans}{OMS}{cmbrs}{m}{n}
%\SetSymbolFont{symbols}     {sans}{OMS}{jkp}  {m}{n}
% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{symbols}{sans}{LMS}{ntxsy}{m}{n}
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
%\DeclareSymbolFont{extrasymbols}  {OMS}{cmbrs}{m}{n}
%\SetSymbolFont{extrasymbols}{sans}{OMS}{cmbrs}{m}{n}
% Some symbols (e.g., \prime) look weird in kpfonts.
% This provides the option to replace them by symbols from mathdesign-charter.

\SetMathAlphabet{\mathit} {normal}{T1}{\savermfamily}{\savermmdseries}{it}
\SetMathAlphabet{\mathit} {bold}  {T1}{\savermfamily}{\savermbfseries}{it}

\SetMathAlphabet{\mathit} {sans}{T1}{\savesffamily}{\savesfmdseries}{it}
\SetMathAlphabet{\mathbf} {sans}{T1}{\savesffamily}{\savesfbfseries}{n}
\SetMathAlphabet{\mathtt} {sans}{OT1}{cmtl}{m}{n}
\SetMathAlphabet{\mathcal}{sans}{LMS}{ntxsy}{m}{n}
% See https://tex.stackexchange.com/questions/231583/import-mathcal-symbols-from-txfonts
%\SetSymbolFont{largesymbols}{sans}{OMX}{jkpss}{m}{n}
%	% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{largesymbols} {sans}{OMX}{mdbch}{m}{n}
% Using symbols like \int, \left(, etc. from mathdesign-charter because they look better than the ones included in kpfonts
% Using symbols like \int, \left(, etc. from newtxmath:
%\DeclareSymbolFont{largesymbols}{LMX}{ntxexx}{m}{n}
\SetSymbolFont{largesymbols}{sans}{LMX}{ntxexx}{m}{n}

\DeclareMathVersion{sansup}
%\SetSymbolFont{letters}  {sansup}{OML}{jkpss}{m}{it}
%\SetSymbolFont{symbols}  {sansup}{OMS}{jkp}  {m}{n}
%\SetSymbolFont{symbols}{sansup}{LMS}{ntxsy}{m}{n}
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty

\DeclareMathVersion{boldsans}
%\SetSymbolFont{operators}{boldsans}{OT1}{jkpss}{b}{n}
%	% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{operators}{boldsans}{OT1}{ntxtlf}{bx}{n}
%\SetSymbolFont{letters}  {boldsans}{OML}{jkpss}{bx}{it}
% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{letters}  {boldsans}{OML}{mdbch}{bx}{it}
%\SetSymbolFont{letters}{boldsans}{OML}{cmbrm}{b}{it}
%\SetSymbolFont{symbols}  {boldsans}{OMS}{jkp}  {bx}{n}
% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
\SetSymbolFont{letters} {boldsans}{OML}{nxlmi} {b}{it}
\SetSymbolFont{lettersA}{boldsans}{U}  {ntxmia}{b}{it}
\SetSymbolFont{symbols} {boldsans}{LMS}{ntxsy} {b}{n}
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
%\SetMathAlphabet{\mathrm}{boldsans}{OT1}{\savesffamily}{\savesfbfseries}{n}
\SetMathAlphabet{\mathit} {boldsans}{T1}{\savesffamily}{\savesfbfseries}{it}
\SetMathAlphabet{\mathtt} {boldsans}{T1}{cmtl}{b}{n}
\SetMathAlphabet{\mathcal}{boldsans}{LMS}{ntxsy}{b}{n}
%\SetSymbolFont{largesymbols}{boldsans}{OMX}{jkpss}{bx}{n}
%	% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{largesymbols}{boldsans}{OMX}{mdbch}{bx}{n}
% Using symbols like \int, \left(, etc. from mathdesign-charter because they look better than the ones included in kpfonts
% Using symbols like \int, \left(, etc. from newtxmath:
\SetSymbolFont{largesymbols}{boldsans}{LMX}{ntxexx}{b}{n}

\DeclareMathVersion{boldsansup}
%\SetSymbolFont{letters}{boldsansup}{OML}{jkpss}{bx}{it}
%\SetSymbolFont{symbols}{boldsansup}{OMS}{jkp}  {bx}{n}
\SetSymbolFont{letters} {boldsans}  {OML}{nxlmi} {b}{it}
\SetSymbolFont{lettersA}{boldsansup}{U}  {ntxmia}{b}{it}
\SetSymbolFont{symbols} {boldsansup}{LMS}{ntxsy} {b}{n}
\SetSymbolFont{lettersA}{normalup}  {U}  {ntxmia}{m}{it}
\SetSymbolFont{lettersA}{boldup}    {U}  {ntxmia}{b}{it}
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
	% Upright Greek characters are taken from the lettersA font.

% Using glyphs for math mode from the custom sansserif font
\DeclareSymbolFont{uprightglyphs}{T1}{\savermfamily}{\savermmdseries}{n}
%\DeclareSymbolFontAlphabet{\mathrm}{uprightglyphs}
%\SetMathAlphabet{\mathrm}{normal}{OT1}{\savermfamily}{\savermmdseries}{n}
\SetSymbolFont{uprightglyphs}{normal}    {T1}{\savermfamily}{\savermmdseries}{n}
\SetSymbolFont{uprightglyphs}{normalup}  {T1}{\savermfamily}{\savermmdseries}{n}
\SetSymbolFont{uprightglyphs}{bold}      {T1}{\savermfamily}{\savermbfseries}{n}
\SetSymbolFont{uprightglyphs}{boldup}    {T1}{\savermfamily}{\savermbfseries}{n}
\SetSymbolFont{uprightglyphs}{sans}      {T1}{\savesffamily}{\savesfmdseries}{n}
\SetSymbolFont{uprightglyphs}{sansup}    {T1}{\savesffamily}{\savesfmdseries}{n}
\SetSymbolFont{uprightglyphs}{boldsans}  {T1}{\savesffamily}{\savesfbfseries}{n}
\SetSymbolFont{uprightglyphs}{boldsansup}{T1}{\savesffamily}{\savesfbfseries}{n}
\DeclareSymbolFont{italicglyphs} {T1}{\savermfamily}{\savermmdseries}{it}
\SetSymbolFont{italicglyphs} {normal}    {T1}{\savermfamily}{\savermmdseries}{it}
\SetSymbolFont{italicglyphs} {normalup}  {T1}{\savermfamily}{\savermmdseries}{n}
\SetSymbolFont{italicglyphs} {bold}      {T1}{\savermfamily}{\savermbfseries}{it}
\SetSymbolFont{italicglyphs} {boldup}    {T1}{\savermfamily}{\savermbfseries}{n}
\SetSymbolFont{italicglyphs} {sans}      {T1}{\savesffamily}{\savesfmdseries}{it}
\SetSymbolFont{italicglyphs} {sansup}    {T1}{\savesffamily}{\savesfmdseries}{n}
\SetSymbolFont{italicglyphs} {boldsans}  {T1}{\savesffamily}{\savesfbfseries}{it}
\SetSymbolFont{italicglyphs} {boldsansup}{T1}{\savesffamily}{\savesfbfseries}{n}

% Syntax of \DeclareMathSymobl:
% \DeclareMathSymbol {<symbol>} {<type>} {<sym-font>} {<slot>}
% Type              Meaning	            Example
% 0 or \mathord     Ordinary             $\alpha$
% 1 or \mathop      Large operator       $\sum$
% 2 or \mathbin     Binary operation     $\times$
% 3 or \mathrel     Relation             $\leq$
% 4 or \mathopen    Opening              $\langle$
% 5 or \mathclose   Closing              $\rangle$
% 6 or \mathpunct   Punctuation          ;
% 7 or \mathalpha   Alphabet character   A
% Example declaration:
% \DeclareMathSymbol{b}{0}{letters}{`b}

% Digits
\DeclareMathSymbol{0}{\mathalpha}{uprightglyphs}{`0}
\DeclareMathSymbol{1}{\mathalpha}{uprightglyphs}{`1}
\DeclareMathSymbol{2}{\mathalpha}{uprightglyphs}{`2}
\DeclareMathSymbol{3}{\mathalpha}{uprightglyphs}{`3}
\DeclareMathSymbol{4}{\mathalpha}{uprightglyphs}{`4}
\DeclareMathSymbol{5}{\mathalpha}{uprightglyphs}{`5}
\DeclareMathSymbol{6}{\mathalpha}{uprightglyphs}{`6}
\DeclareMathSymbol{7}{\mathalpha}{uprightglyphs}{`7}
\DeclareMathSymbol{8}{\mathalpha}{uprightglyphs}{`8}
\DeclareMathSymbol{9}{\mathalpha}{uprightglyphs}{`9}
% Operators and punctuation
%\DeclareMathSymbol{+}{\mathbin}  {operators}    {`+}
%\DeclareMathSymbol{+}{\mathbin}{symbols}{207}
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
% Not from uprightglyphs due to bad spacing
%\DeclareMathSymbol{=}{\mathrel}  {operators}    {`=}
% Not from uprightglyphs due to bad spacing
\DeclareMathSymbol{-}{\mathbin}{symbols}{0}
\DeclareMathSymbol{\leq}{\mathrel}{symbols}{20}
%   \let\le=\leq
\DeclareMathSymbol{\geq}{\mathrel}{symbols}{21}
%   \let\ge=\geq
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
\DeclareMathSymbol{.}{\mathord}  {uprightglyphs}{`.}
\DeclareMathSymbol{,}{\mathpunct}{uprightglyphs}{`,}
\DeclareMathSymbol{:}{\mathrel}  {uprightglyphs}{`:}
\let\colon\relax
\DeclareMathSymbol{\colon}{\mathpunct}{uprightglyphs}{`;}
\DeclareMathSymbol{;}{\mathpunct}{uprightglyphs}{`;}
\DeclareMathSymbol{/}{\mathord}  {uprightglyphs}{`/}
%\DeclareMathSymbol{/}{\mathop}   {uprightglyphs}{`/}
%	% This would icrease the spacing around the division slash slightly
\DeclareMathSymbol{!}{\mathord}  {uprightglyphs}{`!}
\DeclareMathSymbol{\mathdollar}{\mathord}{uprightglyphs}{`\$}
\DeclareRobustCommand{\$}{\ifmmode\mathdollar\else\symbol{`\$}\fi}
\DeclareMathSymbol{\mathpercent}{\mathord}{uprightglyphs}{`\%}
\DeclareRobustCommand{\%}{\ifmmode\mathpercent\else\symbol{`\%}\fi}
\DeclareMathSymbol{&}{\mathbin}{uprightglyphs}{`&}
%\DeclareMathSymbol{(}{\mathopen} {uprightglyphs}{`(}
%\DeclareMathSymbol{)}{\mathclose}{uprightglyphs}{`)}
%\DeclareMathSymbol{[}{\mathopen} {uprightglyphs}{`[}
%\DeclareMathSymbol{]}{\mathclose}{uprightglyphs}{`]}
%\DeclareMathSymbol{\prime}{\mathord}{extrasymbols}{"30}
% Use \prime from mathdesign-charter because it looks better than the one in kpfonts
\DeclareMathDelimiter{(}      {\mathopen} {uprightglyphs}{`(} {largesymbols}{"00}
\DeclareMathDelimiter{)}      {\mathclose}{uprightglyphs}{`)} {largesymbols}{"01}
\DeclareMathDelimiter{[}      {\mathopen} {uprightglyphs}{`[} {largesymbols}{"02}
\DeclareMathDelimiter{]}      {\mathclose}{uprightglyphs}{`]} {largesymbols}{"03}
\DeclareMathDelimiter{\lbrace}{\mathopen} {uprightglyphs}{`\{}{largesymbols}{"08}
\DeclareMathDelimiter{\rbrace}{\mathclose}{uprightglyphs}{`\}}{largesymbols}{"09}
% Uppercase Latin characters
\DeclareMathSymbol{A}{\mathalpha}{italicglyphs}{`A}
\DeclareMathSymbol{B}{\mathalpha}{italicglyphs}{`B}
\DeclareMathSymbol{C}{\mathalpha}{italicglyphs}{`C}
\DeclareMathSymbol{D}{\mathalpha}{italicglyphs}{`D}
\DeclareMathSymbol{E}{\mathalpha}{italicglyphs}{`E}
\DeclareMathSymbol{F}{\mathalpha}{italicglyphs}{`F}
\DeclareMathSymbol{G}{\mathalpha}{italicglyphs}{`G}
\DeclareMathSymbol{H}{\mathalpha}{italicglyphs}{`H}
\DeclareMathSymbol{I}{\mathalpha}{italicglyphs}{`I}
\DeclareMathSymbol{J}{\mathalpha}{italicglyphs}{`J}
\DeclareMathSymbol{K}{\mathalpha}{italicglyphs}{`K}
\DeclareMathSymbol{L}{\mathalpha}{italicglyphs}{`L}
\DeclareMathSymbol{M}{\mathalpha}{italicglyphs}{`M}
\DeclareMathSymbol{N}{\mathalpha}{italicglyphs}{`N}
\DeclareMathSymbol{O}{\mathalpha}{italicglyphs}{`O}
\DeclareMathSymbol{P}{\mathalpha}{italicglyphs}{`P}
\DeclareMathSymbol{Q}{\mathalpha}{italicglyphs}{`Q}
\DeclareMathSymbol{R}{\mathalpha}{italicglyphs}{`R}
\DeclareMathSymbol{S}{\mathalpha}{italicglyphs}{`S}
\DeclareMathSymbol{T}{\mathalpha}{italicglyphs}{`T}
\DeclareMathSymbol{U}{\mathalpha}{italicglyphs}{`U}
\DeclareMathSymbol{V}{\mathalpha}{italicglyphs}{`V}
\DeclareMathSymbol{W}{\mathalpha}{italicglyphs}{`W}
\DeclareMathSymbol{X}{\mathalpha}{italicglyphs}{`X}
\DeclareMathSymbol{Y}{\mathalpha}{italicglyphs}{`Y}
\DeclareMathSymbol{Z}{\mathalpha}{italicglyphs}{`Z}
% lowercase Latin characters
\DeclareMathSymbol{a}{\mathalpha}{italicglyphs}{`a}
\DeclareMathSymbol{b}{\mathalpha}{italicglyphs}{`b}
\DeclareMathSymbol{c}{\mathalpha}{italicglyphs}{`c}
\DeclareMathSymbol{d}{\mathalpha}{italicglyphs}{`d}
\DeclareMathSymbol{e}{\mathalpha}{italicglyphs}{`e}
\DeclareMathSymbol{f}{\mathalpha}{italicglyphs}{`f}
\DeclareMathSymbol{g}{\mathalpha}{italicglyphs}{`g}
\DeclareMathSymbol{h}{\mathalpha}{italicglyphs}{`h}
\DeclareMathSymbol{i}{\mathalpha}{italicglyphs}{`i}
\DeclareMathSymbol{\imath}{\mathalpha}{italicglyphs}{"19}
\DeclareMathSymbol{j}{\mathalpha}{italicglyphs}{`j}
\DeclareMathSymbol{\jmath}{\mathalpha}{italicglyphs}{"1A}
\DeclareMathSymbol{k}{\mathalpha}{italicglyphs}{`k}
\DeclareMathSymbol{l}{\mathalpha}{italicglyphs}{`l}
\DeclareMathSymbol{m}{\mathalpha}{italicglyphs}{`m}
\DeclareMathSymbol{n}{\mathalpha}{italicglyphs}{`n}
\DeclareMathSymbol{o}{\mathalpha}{italicglyphs}{`o}
\DeclareMathSymbol{p}{\mathalpha}{italicglyphs}{`p}
\DeclareMathSymbol{q}{\mathalpha}{italicglyphs}{`q}
\DeclareMathSymbol{r}{\mathalpha}{italicglyphs}{`r}
\DeclareMathSymbol{s}{\mathalpha}{italicglyphs}{`s}
\DeclareMathSymbol{t}{\mathalpha}{italicglyphs}{`t}
\DeclareMathSymbol{u}{\mathalpha}{italicglyphs}{`u}
\DeclareMathSymbol{v}{\mathalpha}{italicglyphs}{`v}
\DeclareMathSymbol{w}{\mathalpha}{italicglyphs}{`w}
\DeclareMathSymbol{x}{\mathalpha}{italicglyphs}{`x}
\DeclareMathSymbol{y}{\mathalpha}{italicglyphs}{`y}
\DeclareMathSymbol{z}{\mathalpha}{italicglyphs}{`z}

% Redefine \cdots so that its appearance matches \ldots, \ddots, and \vdots:
%%% Use math italic, not text, version of dot, in \vdots and \ddots definitions
\makeatletter
\def\cdots{\mathinner{\mkern1mu\raise2.5\p@
    \vbox{\kern7\p@\hbox{$\m@th.$}}\mkern4mu
    \raise2.5\p@\hbox{$\m@th.$}\mkern4mu\raise2.5\p@\hbox{$\m@th.$}\mkern1mu}}
    % \raise2.5\p@ instead of \raise4\p@ to match \cdot
    % \mkern4mu  instead of \mkern2mu  to match \ldots
% Inspired by:
% \def\ddots{\mathinner{\mkern1mu\raise7\p@
%     \vbox{\kern7\p@\hbox{$\m@th.$}}\mkern2mu
%     \raise4\p@\hbox{$\m@th.$}\mkern2mu\raise\p@\hbox{$\m@th.$}\mkern1mu}}
\makeatother
	% Based on http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
%% Sansserif Greek letters
%\DeclareSymbolFont{lgrgreek}{LGR}{\savesffamily}{\savesfmdseries}{it}
%\SetSymbolFont{lgrgreek}{sans}    {LGR}{\savesffamily}{\savesfmdseries}{it}
%\SetSymbolFont{lgrgreek}{boldsans}{LGR}{\savesffamily}{\savesfbfseries}{it}

% The following is taken from
% https://tex.stackexchange.com/questions/116389/automatic-upright-math-when-text-is-in-italic/116399#116399
% Filling in ``missing'' Greek glyphs for completeness
% (not really necessary, since they look identical to Latin glyphs and are thus almost never used)
% ==>
\newcommand{\omicron}{o}
\newcommand{\Digamma}{F}
\newcommand{\Alpha}  {A}
\newcommand{\Beta}   {B}
\newcommand{\Epsilon}{E}
\newcommand{\Zeta}   {Z}
\newcommand{\Eta}    {H}
\newcommand{\Iota}   {I}
\newcommand{\Kappa}  {K}
\newcommand{\Mu}     {M}
\newcommand{\Nu}     {N}
\newcommand{\Omicron}{O}
\newcommand{\Rho}    {P}
\newcommand{\Tau}    {T}
\newcommand{\Chi}    {X}
\newcommand{\omicronup}{\mathup{o}}
\newcommand{\Digammaup}{\mathup{F}}
\newcommand{\Alphaup}  {\mathup{A}}
\newcommand{\Betaup}   {\mathup{B}}
\newcommand{\Epsilonup}{\mathup{E}}
\newcommand{\Zetaup}   {\mathup{Z}}
\newcommand{\Etaup}    {\mathup{H}}
\newcommand{\Iotaup}   {\mathup{I}}
\newcommand{\Kappaup}  {\mathup{K}}
\newcommand{\Muup}     {\mathup{M}}
\newcommand{\Nuup}     {\mathup{N}}
\newcommand{\Omicronup}{\mathup{O}}
\newcommand{\Rhoup}    {\mathup{P}}
\newcommand{\Tauup}    {\mathup{T}}
\newcommand{\Chiup}    {\mathup{X}}
% <==

% Save original definitions of the Greek letters
% ==>
\makeatletter
\@for\@tempa:=%
	alpha,beta,gamma,delta,epsilon,varepsilon,zeta,eta,theta,vartheta,iota,kappa,lambda,mu,nu,xi,%
	omicron,pi,varpi,rho,varrho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
	Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
	Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
\do{%
	\expandafter\let\csname\@tempa orig\expandafter\endcsname\csname\@tempa\endcsname%
	\expandafter\let\csname\@tempa uporig\expandafter\endcsname\csname\@tempa up\endcsname%
}%
\makeatother
% <==

% LGR-encoded Greek letters
% ==>
\newcommand{\textformath}[1]{%
	\IfInBoldMode%
	\IfInUpMode\textbf{#1}\else\textit{\bfseries #1}\fi\relax%
	\else
	\IfInUpMode\textup{#1}\else\textit{#1}\fi\relax%
	\fi\relax%
}
% The double curly braces in this section are necessary to be able to use Greek letters
% in subscripts and superscripts without having to enclose theme in curly braces;
% for example, $\sigma_\epsilon$ instead of $\sigma_{\epsilon}$.
% Uppercase
\newcommand{\AlphaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont A}}}}
\newcommand{\BetaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont B}}}}
\newcommand{\GammaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont G}}}}
\newcommand{\DeltaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont D}}}}
\newcommand{\EpsilonLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont E}}}}
\newcommand{\ZetaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont Z}}}}
\newcommand{\EtaLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont H}}}}
\newcommand{\ThetaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont J}}}}
\newcommand{\IotaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont I}}}}
\newcommand{\KappaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont K}}}}
\newcommand{\LambdaLGR}  {{\mathord{\textformath{\fontencoding{LGR}\selectfont L}}}}
\newcommand{\MuLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont M}}}}
\newcommand{\NuLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont N}}}}
\newcommand{\XiLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont X}}}}
\newcommand{\OmicronLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont O}}}}
\newcommand{\PiLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont P}}}}
\newcommand{\RhoLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont R}}}}
\newcommand{\SigmaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont S}}}}
\newcommand{\TauLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont T}}}}
\newcommand{\UpsilonLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont U}}}}
\newcommand{\PhiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont F}}}}
\newcommand{\ChiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont Q}}}}
\newcommand{\PsiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont Y}}}}
\newcommand{\OmegaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont W}}}}
\newcommand{\DigammaLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont \char195}}}}
% lowercase
\newcommand{\alphaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont a}}}}
\newcommand{\betaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont b}}}}
\newcommand{\gammaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont g}}}}
\newcommand{\deltaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont d}}}}
\newcommand{\epsilonLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont e}}}}
\newcommand{\zetaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont z}}}}
\newcommand{\etaLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont h}}}}
\newcommand{\thetaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont j}}}}
\newcommand{\iotaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont i}}}}
\newcommand{\kappaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont k}}}}
\newcommand{\lambdaLGR}  {{\mathord{\textformath{\fontencoding{LGR}\selectfont l}}}}
\newcommand{\muLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont m}}}}
\newcommand{\nuLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont n}}}}
\newcommand{\xiLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont x}}}}
\newcommand{\omicronLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont o}}}}
\newcommand{\piLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont p}}}}
\newcommand{\rhoLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont r}}}}
\newcommand{\sigmaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont s\noboundary}}}}
% \noboundary prevents sigma from being replaced by the word-end sigma (varsigma),
% see http://mirrors.ctan.org/macros/latex/contrib/textgreek/textgreek.pdf
\newcommand{\varsigmaLGR}{{\mathord{\textformath{\fontencoding{LGR}\selectfont c}}}}
\newcommand{\tauLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont t}}}}
\newcommand{\upsilonLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont u}}}}
\newcommand{\phiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont f}}}}
\newcommand{\chiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont q}}}}
\newcommand{\psiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont y}}}}
\newcommand{\omegaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont w}}}}
\newcommand{\digammaLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont \char147}}}}
% Uppercase, upright
\newcommand{\AlphaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont A}}}}
\newcommand{\BetaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont B}}}}
\newcommand{\GammaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont G}}}}
\newcommand{\DeltaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont D}}}}
\newcommand{\EpsilonupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont E}}}}
\newcommand{\ZetaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont Z}}}}
\newcommand{\EtaupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont H}}}}
\newcommand{\ThetaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont J}}}}
\newcommand{\IotaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont I}}}}
\newcommand{\KappaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont K}}}}
\newcommand{\LambdaupLGR}  {{\mathord{\textup{\fontencoding{LGR}\selectfont L}}}}
\newcommand{\MuupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont M}}}}
\newcommand{\NuupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont N}}}}
\newcommand{\XiupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont X}}}}
\newcommand{\OmicronupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont O}}}}
\newcommand{\PiupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont P}}}}
\newcommand{\RhoupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont R}}}}
\newcommand{\SigmaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont S}}}}
\newcommand{\TauupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont T}}}}
\newcommand{\UpsilonupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont U}}}}
\newcommand{\PhiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont F}}}}
\newcommand{\ChiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont Q}}}}
\newcommand{\PsiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont Y}}}}
\newcommand{\OmegaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont W}}}}
\newcommand{\DigammaupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont \char195}}}}
% lowercase, upright
\newcommand{\alphaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont a}}}}
\newcommand{\betaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont b}}}}
\newcommand{\gammaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont g}}}}
\newcommand{\deltaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont d}}}}
\newcommand{\epsilonupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont e}}}}
\newcommand{\zetaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont z}}}}
\newcommand{\etaupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont h}}}}
\newcommand{\thetaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont j}}}}
\newcommand{\iotaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont i}}}}
\newcommand{\kappaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont k}}}}
\newcommand{\lambdaupLGR}  {{\mathord{\textup{\fontencoding{LGR}\selectfont l}}}}
\newcommand{\muupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont m}}}}
\newcommand{\nuupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont n}}}}
\newcommand{\xiupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont x}}}}
\newcommand{\omicronupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont o}}}}
\newcommand{\piupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont p}}}}
\newcommand{\rhoupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont r}}}}
\newcommand{\sigmaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont s\noboundary}}}}
% \noboundary prevents sigma from being replaced by the word-end sigma (varsigma),
% see http://mirrors.ctan.org/macros/latex/contrib/textgreek/textgreek.pdf
\newcommand{\varsigmaupLGR}{{\mathord{\textup{\fontencoding{LGR}\selectfont c}}}}
\newcommand{\tauupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont t}}}}
\newcommand{\upsilonupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont u}}}}
\newcommand{\phiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont f}}}}
\newcommand{\chiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont q}}}}
\newcommand{\psiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont y}}}}
\newcommand{\omegaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont w}}}}
\newcommand{\digammaupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont \char147}}}}
% <==

% Based on description of the TS1 encoding in
% http://ctan.math.illinois.edu/macros/latex/doc/encguide.pdf:
%\let \oldpm    \pm
%\let \oldtimes \times
%\let \olddiv   \div
%\makeatletter
%\newcommand{\pmsf}   {\mathbin{\text{\usefont{TS1}{\sfdefault}{\f@series}{n}\char"B1}}}
%\newcommand{\timessf}{\mathbin{\text{\usefont{TS1}{\sfdefault}{\f@series}{n}\char"D6}}}
%\newcommand{\divsf}  {\mathbin{\text{\usefont{TS1}{\sfdefault}{\f@series}{n}\char"F6}}}
%\makeatother

% Use LGR-encoded Greek letters for \mathversion{sans}
% ==>
\makeatletter

% Save original definition of \varepsilon etc.
\@for\@tempa:=%
	epsilon,theta,pi,rho,sigma,phi%
\do{%
	\expandafter\let\csname var\@tempa orig\expandafter\endcsname\csname var\@tempa\endcsname%
}

\newcommand*{\sansmath}{%
	\@for\@tempa:=%
		alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
		omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
		Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
		Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa LGR\endcsname%
		\expandafter\let\csname\@tempa up\expandafter\endcsname\csname\@tempa upLGR\endcsname%
		\expandafter\let\csname up\@tempa\expandafter\endcsname\csname\@tempa upLGR\endcsname%
	}%
	\@for\@tempa:=%
		epsilon,theta,pi,rho,phi%
	\do{%
		\expandafter\let\csname var\@tempa\expandafter\endcsname\csname\@tempa\endcsname%
		\expandafter\let\csname var\@tempa up\expandafter\endcsname\csname\@tempa up\endcsname%
		\expandafter\let\csname upvar\@tempa\expandafter\endcsname\csname up\@tempa\endcsname%
	}%
	%\renewcommand{\pm}{\pmsf}%
	%\renewcommand{\times}{\timessf}%
	%\renewcommand{\div}{\divsf}%
}
% <==

% Switch back to the original Greek letters for \mathversion{normal}, i.e., the serif font
% ==>
\newcommand*{\unsansmath}{%
	\@for\@tempa:=%
		alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
		omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
		Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
		Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa orig\endcsname%
		\expandafter\let\csname\@tempa up\expandafter\endcsname\csname\@tempa uporig\endcsname%
		\expandafter\let\csname up\@tempa\expandafter\endcsname\csname\@tempa uporig\endcsname%
	}%
	\@for\@tempa:=%
		epsilon,theta,pi,rho,phi%
	\do{%
		\expandafter\let\csname var\@tempa\expandafter\endcsname\csname var\@tempa orig\endcsname%
		\expandafter\let\csname var\@tempa up\expandafter\endcsname\csname var\@tempa uporig\endcsname%
		\expandafter\let\csname upvar\@tempa\expandafter\endcsname\csname var\@tempa uporig\endcsname%
	}%
	%\renewcommand{\pm}{\oldpm}%
	%\renewcommand{\times}{\oldtimes}%
	%\renewcommand{\div}{\olddiv}%
}
% <==

%% If you would like to use LGR-encoded Greek letters also for the serif font
%% ==>
%\renewcommand*{\unsansmath}{%
%	\@for\@tempa:=%
%		alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
%		omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
%		Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
%		Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
%		\do{%
%			\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa LGR\endcsname%
%			\expandafter\let\csname\@tempa up\expandafter\endcsname\csname\@tempa upLGR\endcsname%
%			\expandafter\let\csname up\@tempa\expandafter\endcsname\csname\@tempa upLGR\endcsname%
%		}%
%	%\renewcommand{\pm}{\pmsf}%
%	%\renewcommand{\times}{\timessf}%
%	%\renewcommand{\div}{\divsf}%
%}
%% <==

\newcommand*{\upgreekletters}{%
	\@for\@tempa:=%
		alpha,beta,gamma,delta,epsilon,varepsilon,zeta,eta,theta,vartheta,iota,kappa,lambda,mu,nu,xi,%
		omicron,pi,varpi,rho,varrho,sigma,varsigma,tau,upsilon,phi,varphi,chi,psi,omega,digamma,%
		Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
		Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa up\endcsname%
	}%
}
\newcommand*{\itgreekletters}{%
	\@for\@tempa:=%
		alpha,beta,gamma,delta,epsilon,varepsilon,zeta,eta,theta,vartheta,iota,kappa,lambda,mu,nu,xi,%
		omicron,pi,varpi,rho,varrho,sigma,varsigma,tau,upsilon,phi,varphi,chi,psi,omega,digamma,%
		Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
		Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa orig\endcsname%
	}%
}

\makeatother

%\makeatletter
%	\@for\@tempa:=%
%	%alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
%	%pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
%	Gamma,Delta,Theta,Lambda,Xi,Pi,Sigma,Upsilon,Phi,Psi,Omega%
%	\do{\expandafter\let\csname\@tempa\expandafter\endcsname\csname other\@tempa\endcsname}%
%\makeatother

% Fix the \bm command so that it also works properly in the sans mathversions
% ==>
\let \bmorig \bm
\renewcommand{\bm}[1]{%
	\IfInSansMode%
		\textbf{\mathversion{boldsans}\(#1\)}%
	\else%
		{\InBoldModetrue\bmorig{#1}}%
	\fi\relax%
}
% <==
\renewcommand{\mathbf}[1]{\bm{#1}}
\renewcommand{\boldsymbol}[1]{\bm{#1}}
\newcommand{\mathbfit}[1]{\bm{#1}}
%\renewcommand{\mathcal}[1]{\mathscr{#1}}
\renewcommand{\mathscr}[1]{\mathcal{#1}}

% Apply sansmath etc. automagically
% ==>
\newif\IfInSansMode
\newif\IfInBoldMode
\newif\IfInUpMode
\let \oldsf \sffamily
\renewcommand*{\sffamily}{%
	\oldsf\sansmath\InSansModetrue%
	\IfInBoldMode\mathversion{boldsans}\else\mathversion{sans}\fi\relax%
}
\let \oldbf \bfseries
\renewcommand*{\bfseries}{%
	\oldbf\InBoldModetrue%
	\IfInSansMode\sansmath\mathversion{boldsans}\else\mathversion{bold}\fi\relax%
}
\let \oldmd \mdseries
\renewcommand*{\mdseries}{%
	\oldmd\InBoldModefalse%
	\IfInSansMode\sansmath\mathversion{sans}\else\mathversion{normal}\fi\relax%
}
\let \oldnorm \normalfont
\renewcommand*{\normalfont}{%
	\oldnorm\InSansModefalse\InBoldModefalse\mathversion{normal}%
	\unsansmath%
}
\let \oldrm \rmfamily
\renewcommand*{\rmfamily}{%
	\oldrm\InSansModefalse%
	\IfInBoldMode\mathversion{bold}\else\mathversion{normal}\fi\relax%
	\unsansmath%
}
% <==

% Make \mathnormal obey the currently active \mathversion ==>
\let \mathnormalorig \mathnormal
\renewcommand{\mathnormal}[1]{%
	\IfInSansMode%
		\IfInBoldMode%
			\mathversion{boldsans}%
			{\textbf{\(#1\)}}%
		\else%
			\mathversion{sans}%
			{\textmd{\(#1\)}}%
		\fi\relax%
	\else%
		\mathnormalorig{#1}%
	\fi\relax%
}
% <==

% Adjust \mathrm to the curretly active \mathversion.
% We set it up such that also in sansserif mode, \mathrm activates the serif font.
% ==>
%\DeclareMathAlphabet{\mathrm}{OT1}{\savermfamily}{\savermmdseries}{n}
\let \mathrmorig \mathrm
\renewcommand{\mathrm}[1]{%
	\IfInSansMode%
		{\textrm{%
			\IfInBoldMode%
				\mathversion{bold}%
				\(\mathrmorig{#1}\)%
			\else%
				\mathversion{normal}%
				\(\mathrmorig{#1}\)%
			\fi\relax%
		}}%
	\else%
		\mathrmorig{#1}%
	\fi\relax%
}
% <==

% Define \mathup to activate \upshape without switching to the serif font
% (in contrast to \mathrm)
% ==>
\newcommand{\mathup}[1]{%
	\IfInSansMode%
		{\textup{%
			\InUpModetrue%
				\IfInBoldMode%
				\mathversion{boldsansup}%
				\(#1\)%
			\else%
				\mathversion{sansup}%
				\(#1\)%
			\fi\relax%
		}}%
	\else%
		{\upgreekletters\mathrm{#1}\itgreekletters}%
	\fi\relax%
}
\newcommand{\mathbfup}[1]{%
	\mathbf{\mathup{#1}}
}
% <==

% If you would like to redefine \mathup also for the serif font:
% ==>
\renewcommand{\mathup}[1]{%
	\IfInSansMode%
		{\textup{%
			\InUpModetrue%
			\IfInBoldMode%
				\mathversion{boldsansup}%
				\(#1\)%
			\else%
				\mathversion{sansup}%
				\(#1\)%
			\fi\relax%
		}}%
	\else%
		{\textup{%
			\InUpModetrue%
			\upgreekletters%
			\IfInBoldMode%
				\mathversion{boldup}%
				\(#1\)%
			\else%
				\mathversion{normalup}%
				\(#1\)%
			\fi\relax%
		}}%
	\fi\relax%
}
\renewcommand{\mathbfup}[1]{{%
	\InBoldModetrue%
	\IfInSansMode%
		{\mathbf{\mathup{#1}}}%
	\else%
		{\upgreekletters\mathbf{\mathup{#1}}\itgreekletters}%
	\fi\relax%
}}
% <==

%\SetMathAlphabet{\mathrm}{normal}{OT1}{\savermfamily}{\savermmdseries}{n}
%\DeclareMathAlphabet{\mathrm}{OT1}{\savermfamily}{\savermmdseries}{n}
\renewcommand{\mathrm}[1]{%
	{\textup{%
		\protect\InUpModetrue%
		\IfInBoldMode%
			\mathversion{boldup}%
			\protect\upgreekletters%
			\(#1\)%
		\else%
			\mathversion{normalup}%
			\protect\upgreekletters%
			\(#1\)%
		\fi\relax%
	 }}%
}

% Make the LaTeX-defined operators obey sansserif math
% ==>
\let \operatornameorig \operatorname
\renewcommand{\operatorname}[1]{%
	\operatornameorig{\mathup{#1}}%
}
\makeatletter
\@for\@tempa:=%
	arccos,arccot,arccsc,arcsec,arcsin,arctan,arg,cos,cosh,cot,coth,csc,%
	deg,det,dim,exp,gcd,hom,inf,ker,lg,lim,liminf,limsup,ln,log,max,min,%
	Pr,sec,sin,sinh,sup,tan,tanh%
\do{%
	\expandafter\let\csname\@tempa\endcsname\relax%
}%
\makeatother
\DeclareMathOperator {\arccos}{\mathup{arccos}}
\DeclareMathOperator {\arccot}{\mathup{arccot}}
\DeclareMathOperator {\arccsc}{\mathup{arccsc}}
\DeclareMathOperator {\arcsec}{\mathup{arcsec}}
\DeclareMathOperator {\arcsin}{\mathup{arcsin}}
\DeclareMathOperator {\arctan}{\mathup{arctan}}
\DeclareMathOperator {\arg}   {\mathup{arg}}
\DeclareMathOperator {\cos}   {\mathup{cos}}
\DeclareMathOperator {\cosh}  {\mathup{cosh}}
\DeclareMathOperator {\cot}   {\mathup{cot}}
\DeclareMathOperator {\coth}  {\mathup{coth}}
\DeclareMathOperator {\csc}   {\mathup{csc}}
\DeclareMathOperator {\deg}   {\mathup{deg}}
\DeclareMathOperator {\det}   {\mathup{det}}
\DeclareMathOperator {\dim}   {\mathup{dim}}
\DeclareMathOperator {\exp}   {\mathup{exp}}
\DeclareMathOperator {\gcd}   {\mathup{gcd}}
\DeclareMathOperator*{\hom}   {\mathup{hom}}
\DeclareMathOperator*{\inf}   {\mathup{inf}}
\DeclareMathOperator {\ker}   {\mathup{ker}}
\DeclareMathOperator {\lg}    {\mathup{lg}}
\DeclareMathOperator {\lim}   {\mathup{lim}}
\DeclareMathOperator*{\liminf}{\mathup{lim\,inf}}
\DeclareMathOperator*{\limsup}{\mathup{lim\,sup}}
\DeclareMathOperator {\ln}    {\mathup{ln}}
\DeclareMathOperator {\log}   {\mathup{log}}
\DeclareMathOperator*{\max}   {\mathup{max}}
\DeclareMathOperator*{\min}   {\mathup{min}}
\DeclareMathOperator {\Pr}    {\mathup{Pr}}
\DeclareMathOperator {\sec}   {\mathup{sec}}
\DeclareMathOperator {\sin}   {\mathup{sin}}
\DeclareMathOperator {\sinh}  {\mathup{sinh}}
\DeclareMathOperator*{\sup}   {\mathup{sup}}
\DeclareMathOperator {\tan}   {\mathup{tan}}
\DeclareMathOperator {\tanh}  {\mathup{tanh}}
% <==

==> 0_0_Preamble/johannes_chess_commands.tex <==
% !TeX program = pdflatex
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !BIB program = biber
% !TeX TXS-program:bibliography = txs:///biber


%\usepackage{stackengine}
%\setstackgap{S}{0pt}
\usepackage{booktabs,dcolumn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FUNDAMENTAL PACKAGES AND COMMANDS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% CHESS
\usepackage{threeparttable}

\newcommand\Pairtwo[4]{%
	\begin{footnotesize}
		\begin{tabular}{|p{1.5cm}|p{0.5cm}p{0.5cm}|}
			\hline
			#1 \\
			\hline Guten
			#2  \\
			\hline
			#3 \\
			\hline
			#4 \\
			\hline
		\end{tabular}%
	\end{footnotesize}
}


\newcommand\Pairfour[4]{%
	\begin{footnotesize}
		\begin{tabular}{|p{1.5cm}|p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}|}
			\hline
			#1 \\
			\hline 
			#2  \\
			\hline
			#3 \\
			\hline
			#4 \\
			\hline
		\end{tabular}%
	\end{footnotesize}
}



\newcommand\Pairsix[4]{%
	\begin{footnotesize}
		\begin{tabular}{|p{1.5cm}|p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}|}
			\hline
			#1 \\
			\hline 
			#2  \\
			\hline
			#3 \\
			\hline
			#4 \\
			\hline
		\end{tabular}%
	\end{footnotesize}
}



\newcommand{\tablenotetext}{\textit{Note:} Standard errors clustered on the game-level in parentheses. The sample consists of World Cup games from 2013 -- 2023. The dependent variable varies on the half-move-level. As explained in Section \ref{sec:rel_outcomes_strategic_uncertainty}, it is computed as the logarithm of the variance over the difficulties of the hypothetical boards that can arise after the played move. \textit{Remaining Time} is instrumented with the interaction of half-move dummies and initial thinking time of the specific time control. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01}




%\usepackage{yhmath}
%\stackMath
%\newcommand\reallywidehat[1]{%
%	\savestack{\tmpbox}{\stretchto{%
%			\scaleto{%
%				\scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
%				{\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
%			}{\textheight}%
%		}{0.5ex}}%
%	\stackon[1pt]{#1}{\tmpbox}%
%}
\parskip 1ex
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}



\newcommand\citeposs[1]{\citeauthor{#1}'s\ \citeyear{#1}}

\newcolumntype{d}[1]{D{.}{.}{#1}}
\newcommand{\mc}{\multicolumn}

\setlength{\parskip}{12pt}
\setlength\parindent{12pt}

\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bbeta}{\boldsymbol{\beta}}

\newlength\myboxwidth
\setlength{\myboxwidth}{\dimexpr\textwidth-2\fboxsep}




\newcommand\blfootnote[1]{%
	\begingroup
	\renewcommand\thefootnote{}\footnote{#1}%
	\addtocounter{footnote}{-1}%
	\endgroup
}


\newcommand{\SE}{Standard errors clustered on person level in parentheses. }



\makeatletter
\def\@fnsymbol#1{\ensuremath{\ifcase#1\or *\or \mathsection\or \mathparagraph\or \|\or **\or \dagger\dagger
		\or \ddagger\ddagger \else\@ctrerr\fi}}
\makeatother






==> 1_JMP/002_Abstract.tex <==
\begin{center}
\textbf{Abstract}
\end{center}


{\small \noindent
I study altruistic choices through the lens of a cognitively noisy decision-maker. I introduce a theoretical framework that demonstrates how increased cognitive noise can directionally affect altruistic decisions and put its implications to the test: In a laboratory experiment, participants make a series of binary choices between taking and giving monetary payments. In the treatment, to-be-calculated math sums replace straightforward monetary payments, increasing the cognitive difficulty of choosing. The Treatment group exhibits a lower sensitivity towards changes in payments and decides significantly more often in favor of the other person, i.e., is more altruistic. I explore the origins of this effect with Bayesian hierarchical models and a number-comparison task, mirroring the "mechanics" of the altruism choices absent any altruistic preference. The treatment effect is similar in this task, suggesting that the perception of numerical magnitudes drives treatment differences. The probabilistic model supports this interpretation. A series of additional results show a negative correlation between cognitive reflection and individual measures of cognitive noise, as well as associations between altruistic choice and number comparison. Overall, these results suggest that the expression of altruistic preferences -- and potentially social preferences more generally -- is affected by the cognitive difficulty of their implementation.
}

\keywords{{Cognitive Noise, Altruism, Bayesian Hierarchical Models, Experiment}}

\JEL{{C91, D91}}
\clearpage

==> abstract.tex <==
I study altruistic choices through the lens of a cognitively noisy decision-maker. I introduce a theoretical framework that demonstrates how increased cognitive noise can directionally affect altruistic decisions and put its implications to the test: In a laboratory experiment, participants make a series of binary choices between taking and giving monetary payments. In the treatment, to-be-calculated sums replace plain monetary payments, increasing the cognitive difficulty of choosing. The Treatment group exhibits a lower sensitivity towards changes in payments and decides significantly more often in favor of the other person, i.e., is more altruistic. I explore the origins of this effect with Bayesian hierarchical models and a number-comparison task, mirroring the mechanics of the altruism choices absent any altruistic preference. The treatment effect is similar in this task, suggesting that a biased perception of numerical magnitudes drives treatment differences. The probabilistic models support this conclusion. A series of additional results show a negative correlation between cognitive reflection and individual measures of cognitive noise, as well as associations between altruistic choice and number comparison. Overall, these results suggest that the expression of altruistic preferences -- and potentially social preferences more generally -- is affected by the cognitive difficulty of their implementation.


==> graphs_export/experiment/trials_table.tex <==
\begin{longtable}[t]{rrrrrrrr}
\caption{Overview of 240 trials of the altruism task \label{tab:trials_overview}}\\
\toprule
\multicolumn{2}{c}{Game Identifiers} & \multicolumn{2}{c}{Payments} & \multicolumn{4}{c}{Components of Sums (Treatment)} \\
\cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-4} \cmidrule(l{3pt}r{3pt}){5-8}
Game ID & Game Group & Other & Self & Self 1 & Self 2 & Other 1 & Other 2\\
\midrule
\endfirsthead
\caption[]{Overview of 240 trials of the altruism task  \textit{(continued)}}\\
\toprule
\multicolumn{2}{c}{Game Identifiers} & \multicolumn{2}{c}{Payments} & \multicolumn{4}{c}{Components of Sums (Treatment)} \\
\cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-4} \cmidrule(l{3pt}r{3pt}){5-8}
Game ID & Game Group & Other & Self & Self 1 & Self 2 & Other 1 & Other 2\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
0 & 1 & 655 & 0 & 0 & 0 & 543 & 112\\
0 & 1 & 655 & 0 & 0 & 0 & 629 & 26\\
0 & 1 & 655 & 0 & 0 & 0 & 490 & 165\\
0 & 1 & 655 & 0 & 0 & 0 & 32 & 623\\
0 & 1 & 655 & 0 & 0 & 0 & 540 & 115\\
\addlinespace
1 & 1 & 655 & 34 & 14 & 20 & 638 & 17\\
1 & 1 & 655 & 34 & 23 & 11 & 20 & 635\\
1 & 1 & 655 & 34 & 22 & 12 & 643 & 12\\
1 & 1 & 655 & 34 & 15 & 19 & 14 & 641\\
1 & 1 & 655 & 34 & 22 & 12 & 10 & 645\\
\addlinespace
2 & 1 & 655 & 72 & 24 & 48 & 627 & 28\\
2 & 1 & 655 & 72 & 35 & 37 & 34 & 621\\
2 & 1 & 655 & 72 & 58 & 14 & 26 & 629\\
2 & 1 & 655 & 72 & 61 & 11 & 40 & 615\\
2 & 1 & 655 & 72 & 37 & 35 & 35 & 620\\
\addlinespace
3 & 1 & 655 & 115 & 31 & 84 & 33 & 622\\
3 & 1 & 655 & 115 & 36 & 79 & 621 & 34\\
3 & 1 & 655 & 115 & 39 & 76 & 617 & 38\\
3 & 1 & 655 & 115 & 28 & 87 & 645 & 10\\
3 & 1 & 655 & 115 & 34 & 81 & 585 & 70\\
\addlinespace
4 & 1 & 655 & 163 & 62 & 101 & 11 & 644\\
4 & 1 & 655 & 163 & 12 & 151 & 10 & 645\\
4 & 1 & 655 & 163 & 15 & 148 & 643 & 12\\
4 & 1 & 655 & 163 & 13 & 150 & 643 & 12\\
4 & 1 & 655 & 163 & 140 & 23 & 554 & 101\\
\addlinespace
5 & 1 & 655 & 218 & 167 & 51 & 47 & 608\\
5 & 1 & 655 & 218 & 164 & 54 & 509 & 146\\
5 & 1 & 655 & 218 & 172 & 46 & 622 & 33\\
5 & 1 & 655 & 218 & 81 & 137 & 41 & 614\\
5 & 1 & 655 & 218 & 18 & 200 & 122 & 533\\
\addlinespace
6 & 1 & 655 & 280 & 170 & 110 & 588 & 67\\
6 & 1 & 655 & 280 & 234 & 46 & 60 & 595\\
6 & 1 & 655 & 280 & 90 & 190 & 104 & 551\\
6 & 1 & 655 & 280 & 161 & 119 & 506 & 149\\
6 & 1 & 655 & 280 & 126 & 154 & 15 & 640\\
\addlinespace
7 & 1 & 655 & 352 & 107 & 245 & 557 & 98\\
7 & 1 & 655 & 352 & 161 & 191 & 68 & 587\\
7 & 1 & 655 & 352 & 227 & 125 & 583 & 72\\
7 & 1 & 655 & 352 & 310 & 42 & 645 & 10\\
7 & 1 & 655 & 352 & 170 & 182 & 486 & 169\\
\addlinespace
8 & 1 & 655 & 436 & 68 & 368 & 51 & 604\\
8 & 1 & 655 & 436 & 331 & 105 & 97 & 558\\
8 & 1 & 655 & 436 & 425 & 11 & 485 & 170\\
8 & 1 & 655 & 436 & 326 & 110 & 634 & 21\\
8 & 1 & 655 & 436 & 312 & 124 & 158 & 497\\
\addlinespace
9 & 1 & 655 & 535 & 199 & 336 & 471 & 184\\
9 & 1 & 655 & 535 & 413 & 122 & 71 & 584\\
9 & 1 & 655 & 535 & 398 & 137 & 27 & 628\\
9 & 1 & 655 & 535 & 426 & 109 & 478 & 177\\
9 & 1 & 655 & 535 & 222 & 313 & 443 & 212\\
\addlinespace
10 & 1 & 655 & 655 & 253 & 402 & 79 & 576\\
10 & 1 & 655 & 655 & 277 & 378 & 82 & 573\\
10 & 1 & 655 & 655 & 332 & 323 & 575 & 80\\
10 & 1 & 655 & 655 & 361 & 294 & 565 & 90\\
10 & 1 & 655 & 655 & 156 & 499 & 419 & 236\\
\addlinespace
11 & 1 & 655 & 800 & 740 & 60 & 515 & 140\\
11 & 1 & 655 & 800 & 678 & 122 & 260 & 395\\
11 & 1 & 655 & 800 & 503 & 297 & 635 & 20\\
11 & 1 & 655 & 800 & 311 & 489 & 39 & 616\\
11 & 1 & 655 & 800 & 744 & 56 & 244 & 411\\
\addlinespace
12 & 2 & 926 & 0 & 0 & 0 & 850 & 76\\
12 & 2 & 926 & 0 & 0 & 0 & 836 & 90\\
12 & 2 & 926 & 0 & 0 & 0 & 254 & 672\\
12 & 2 & 926 & 0 & 0 & 0 & 418 & 508\\
12 & 2 & 926 & 0 & 0 & 0 & 391 & 535\\
\addlinespace
13 & 2 & 926 & 48 & 13 & 35 & 10 & 916\\
13 & 2 & 926 & 48 & 11 & 37 & 10 & 916\\
13 & 2 & 926 & 48 & 36 & 12 & 19 & 907\\
13 & 2 & 926 & 48 & 32 & 16 & 26 & 900\\
13 & 2 & 926 & 48 & 30 & 18 & 914 & 12\\
\addlinespace
14 & 2 & 926 & 102 & 84 & 18 & 11 & 915\\
14 & 2 & 926 & 102 & 39 & 63 & 32 & 894\\
14 & 2 & 926 & 102 & 76 & 26 & 909 & 17\\
14 & 2 & 926 & 102 & 35 & 67 & 19 & 907\\
14 & 2 & 926 & 102 & 66 & 36 & 20 & 906\\
\addlinespace
15 & 2 & 926 & 163 & 70 & 93 & 69 & 857\\
15 & 2 & 926 & 163 & 138 & 25 & 28 & 898\\
15 & 2 & 926 & 163 & 111 & 52 & 48 & 878\\
15 & 2 & 926 & 163 & 39 & 124 & 114 & 812\\
15 & 2 & 926 & 163 & 25 & 138 & 17 & 909\\
\addlinespace
16 & 2 & 926 & 231 & 214 & 17 & 16 & 910\\
16 & 2 & 926 & 231 & 62 & 169 & 53 & 873\\
16 & 2 & 926 & 231 & 35 & 196 & 914 & 12\\
16 & 2 & 926 & 231 & 67 & 164 & 864 & 62\\
16 & 2 & 926 & 231 & 161 & 70 & 126 & 800\\
\addlinespace
17 & 2 & 926 & 308 & 90 & 218 & 45 & 881\\
17 & 2 & 926 & 308 & 101 & 207 & 169 & 757\\
17 & 2 & 926 & 308 & 22 & 286 & 905 & 21\\
17 & 2 & 926 & 308 & 84 & 224 & 38 & 888\\
17 & 2 & 926 & 308 & 173 & 135 & 99 & 827\\
\addlinespace
18 & 2 & 926 & 396 & 11 & 385 & 10 & 916\\
18 & 2 & 926 & 396 & 184 & 212 & 733 & 193\\
18 & 2 & 926 & 396 & 74 & 322 & 45 & 881\\
18 & 2 & 926 & 396 & 170 & 226 & 896 & 30\\
18 & 2 & 926 & 396 & 325 & 71 & 187 & 739\\
\addlinespace
19 & 2 & 926 & 498 & 63 & 435 & 51 & 875\\
19 & 2 & 926 & 498 & 264 & 234 & 879 & 47\\
19 & 2 & 926 & 498 & 330 & 168 & 273 & 653\\
19 & 2 & 926 & 498 & 325 & 173 & 779 & 147\\
19 & 2 & 926 & 498 & 366 & 132 & 50 & 876\\
\addlinespace
20 & 2 & 926 & 617 & 486 & 131 & 200 & 726\\
20 & 2 & 926 & 617 & 410 & 207 & 148 & 778\\
20 & 2 & 926 & 617 & 409 & 208 & 775 & 151\\
20 & 2 & 926 & 617 & 416 & 201 & 186 & 740\\
20 & 2 & 926 & 617 & 106 & 511 & 470 & 456\\
\addlinespace
21 & 2 & 926 & 757 & 565 & 192 & 171 & 755\\
21 & 2 & 926 & 757 & 604 & 153 & 106 & 820\\
21 & 2 & 926 & 757 & 480 & 277 & 152 & 774\\
21 & 2 & 926 & 757 & 557 & 200 & 821 & 105\\
21 & 2 & 926 & 757 & 733 & 24 & 470 & 456\\
\addlinespace
22 & 2 & 926 & 926 & 224 & 702 & 647 & 279\\
22 & 2 & 926 & 926 & 79 & 847 & 730 & 196\\
22 & 2 & 926 & 926 & 117 & 809 & 83 & 843\\
22 & 2 & 926 & 926 & 46 & 880 & 727 & 199\\
22 & 2 & 926 & 926 & 370 & 556 & 567 & 359\\
\addlinespace
23 & 2 & 926 & 1132 & 827 & 305 & 711 & 215\\
23 & 2 & 926 & 1132 & 669 & 463 & 146 & 780\\
23 & 2 & 926 & 1132 & 1072 & 60 & 863 & 63\\
23 & 2 & 926 & 1132 & 598 & 534 & 222 & 704\\
23 & 2 & 926 & 1132 & 867 & 265 & 323 & 603\\
\addlinespace
24 & 3 & 1310 & 0 & 0 & 0 & 963 & 347\\
24 & 3 & 1310 & 0 & 0 & 0 & 898 & 412\\
24 & 3 & 1310 & 0 & 0 & 0 & 726 & 584\\
24 & 3 & 1310 & 0 & 0 & 0 & 876 & 434\\
24 & 3 & 1310 & 0 & 0 & 0 & 459 & 851\\
\addlinespace
25 & 3 & 1310 & 68 & 35 & 33 & 1288 & 22\\
25 & 3 & 1310 & 68 & 28 & 40 & 1294 & 16\\
25 & 3 & 1310 & 68 & 31 & 37 & 26 & 1284\\
25 & 3 & 1310 & 68 & 26 & 42 & 10 & 1300\\
25 & 3 & 1310 & 68 & 29 & 39 & 1283 & 27\\
\addlinespace
26 & 3 & 1310 & 145 & 121 & 24 & 1288 & 22\\
26 & 3 & 1310 & 145 & 42 & 103 & 1293 & 17\\
26 & 3 & 1310 & 145 & 79 & 66 & 1286 & 24\\
26 & 3 & 1310 & 145 & 121 & 24 & 1212 & 98\\
26 & 3 & 1310 & 145 & 14 & 131 & 1298 & 12\\
\addlinespace
27 & 3 & 1310 & 231 & 80 & 151 & 1292 & 18\\
27 & 3 & 1310 & 231 & 140 & 91 & 10 & 1300\\
27 & 3 & 1310 & 231 & 34 & 197 & 110 & 1200\\
27 & 3 & 1310 & 231 & 35 & 196 & 28 & 1282\\
27 & 3 & 1310 & 231 & 127 & 104 & 74 & 1236\\
\addlinespace
28 & 3 & 1310 & 327 & 182 & 145 & 1238 & 72\\
28 & 3 & 1310 & 327 & 167 & 160 & 1259 & 51\\
28 & 3 & 1310 & 327 & 62 & 265 & 1257 & 53\\
28 & 3 & 1310 & 327 & 242 & 85 & 1154 & 156\\
28 & 3 & 1310 & 327 & 79 & 248 & 1124 & 186\\
\addlinespace
29 & 3 & 1310 & 436 & 346 & 90 & 1293 & 17\\
29 & 3 & 1310 & 436 & 261 & 175 & 153 & 1157\\
29 & 3 & 1310 & 436 & 112 & 324 & 1233 & 77\\
29 & 3 & 1310 & 436 & 143 & 293 & 215 & 1095\\
29 & 3 & 1310 & 436 & 145 & 291 & 72 & 1238\\
\addlinespace
30 & 3 & 1310 & 561 & 298 & 263 & 1040 & 270\\
30 & 3 & 1310 & 561 & 550 & 11 & 10 & 1300\\
30 & 3 & 1310 & 561 & 202 & 359 & 1254 & 56\\
30 & 3 & 1310 & 561 & 515 & 46 & 934 & 376\\
30 & 3 & 1310 & 561 & 470 & 91 & 884 & 426\\
\addlinespace
31 & 3 & 1310 & 705 & 655 & 50 & 1273 & 37\\
31 & 3 & 1310 & 705 & 442 & 263 & 1161 & 149\\
31 & 3 & 1310 & 705 & 665 & 40 & 278 & 1032\\
31 & 3 & 1310 & 705 & 627 & 78 & 21 & 1289\\
31 & 3 & 1310 & 705 & 597 & 108 & 10 & 1300\\
\addlinespace
32 & 3 & 1310 & 873 & 849 & 24 & 521 & 789\\
32 & 3 & 1310 & 873 & 704 & 169 & 1292 & 18\\
32 & 3 & 1310 & 873 & 758 & 115 & 1271 & 39\\
32 & 3 & 1310 & 873 & 395 & 478 & 62 & 1248\\
32 & 3 & 1310 & 873 & 832 & 41 & 783 & 527\\
\addlinespace
33 & 3 & 1310 & 1071 & 512 & 559 & 416 & 894\\
33 & 3 & 1310 & 1071 & 246 & 825 & 217 & 1093\\
33 & 3 & 1310 & 1071 & 942 & 129 & 72 & 1238\\
33 & 3 & 1310 & 1071 & 493 & 578 & 1262 & 48\\
33 & 3 & 1310 & 1071 & 718 & 353 & 656 & 654\\
\addlinespace
34 & 3 & 1310 & 1310 & 108 & 1202 & 814 & 496\\
34 & 3 & 1310 & 1310 & 63 & 1247 & 1149 & 161\\
34 & 3 & 1310 & 1310 & 750 & 560 & 219 & 1091\\
34 & 3 & 1310 & 1310 & 944 & 366 & 235 & 1075\\
34 & 3 & 1310 & 1310 & 304 & 1006 & 254 & 1056\\
\addlinespace
35 & 3 & 1310 & 1601 & 1045 & 556 & 575 & 735\\
35 & 3 & 1310 & 1601 & 1005 & 596 & 637 & 673\\
35 & 3 & 1310 & 1601 & 1465 & 136 & 800 & 510\\
35 & 3 & 1310 & 1601 & 1459 & 142 & 667 & 643\\
35 & 3 & 1310 & 1601 & 1134 & 467 & 587 & 723\\
\addlinespace
36 & 4 & 1852 & 0 & 0 & 0 & 622 & 1230\\
36 & 4 & 1852 & 0 & 0 & 0 & 1453 & 399\\
36 & 4 & 1852 & 0 & 0 & 0 & 1022 & 830\\
36 & 4 & 1852 & 0 & 0 & 0 & 1110 & 742\\
36 & 4 & 1852 & 0 & 0 & 0 & 734 & 1118\\
\addlinespace
37 & 4 & 1852 & 97 & 85 & 12 & 10 & 1842\\
37 & 4 & 1852 & 97 & 34 & 63 & 27 & 1825\\
37 & 4 & 1852 & 97 & 43 & 54 & 41 & 1811\\
37 & 4 & 1852 & 97 & 27 & 70 & 1828 & 24\\
37 & 4 & 1852 & 97 & 37 & 60 & 54 & 1798\\
\addlinespace
38 & 4 & 1852 & 205 & 54 & 151 & 1740 & 112\\
38 & 4 & 1852 & 205 & 91 & 114 & 1777 & 75\\
38 & 4 & 1852 & 205 & 57 & 148 & 1818 & 34\\
38 & 4 & 1852 & 205 & 83 & 122 & 1785 & 67\\
38 & 4 & 1852 & 205 & 122 & 83 & 113 & 1739\\
\addlinespace
39 & 4 & 1852 & 326 & 216 & 110 & 24 & 1828\\
39 & 4 & 1852 & 326 & 109 & 217 & 198 & 1654\\
39 & 4 & 1852 & 326 & 45 & 281 & 198 & 1654\\
39 & 4 & 1852 & 326 & 64 & 262 & 239 & 1613\\
39 & 4 & 1852 & 326 & 222 & 104 & 81 & 1771\\
\addlinespace
40 & 4 & 1852 & 463 & 74 & 389 & 188 & 1664\\
40 & 4 & 1852 & 463 & 293 & 170 & 77 & 1775\\
40 & 4 & 1852 & 463 & 385 & 78 & 1821 & 31\\
40 & 4 & 1852 & 463 & 150 & 313 & 1706 & 146\\
40 & 4 & 1852 & 463 & 259 & 204 & 171 & 1681\\
\addlinespace
41 & 4 & 1852 & 617 & 367 & 250 & 61 & 1791\\
41 & 4 & 1852 & 617 & 331 & 286 & 1708 & 144\\
41 & 4 & 1852 & 617 & 85 & 532 & 1817 & 35\\
41 & 4 & 1852 & 617 & 414 & 203 & 1838 & 14\\
41 & 4 & 1852 & 617 & 302 & 315 & 277 & 1575\\
\addlinespace
42 & 4 & 1852 & 793 & 50 & 743 & 1358 & 494\\
42 & 4 & 1852 & 793 & 649 & 144 & 42 & 1810\\
42 & 4 & 1852 & 793 & 698 & 95 & 66 & 1786\\
42 & 4 & 1852 & 793 & 431 & 362 & 348 & 1504\\
42 & 4 & 1852 & 793 & 245 & 548 & 142 & 1710\\
\addlinespace
43 & 4 & 1852 & 997 & 239 & 758 & 1188 & 664\\
43 & 4 & 1852 & 997 & 964 & 33 & 960 & 892\\
43 & 4 & 1852 & 997 & 768 & 229 & 1774 & 78\\
43 & 4 & 1852 & 997 & 374 & 623 & 330 & 1522\\
43 & 4 & 1852 & 997 & 772 & 225 & 1442 & 410\\
\addlinespace
44 & 4 & 1852 & 1235 & 1069 & 166 & 1318 & 534\\
44 & 4 & 1852 & 1235 & 1055 & 180 & 759 & 1093\\
44 & 4 & 1852 & 1235 & 103 & 1132 & 1781 & 71\\
44 & 4 & 1852 & 1235 & 715 & 520 & 1516 & 336\\
44 & 4 & 1852 & 1235 & 307 & 928 & 1636 & 216\\
\addlinespace
45 & 4 & 1852 & 1515 & 1276 & 239 & 1119 & 733\\
45 & 4 & 1852 & 1515 & 1276 & 239 & 118 & 1734\\
45 & 4 & 1852 & 1515 & 1237 & 278 & 921 & 931\\
45 & 4 & 1852 & 1515 & 1165 & 350 & 749 & 1103\\
45 & 4 & 1852 & 1515 & 928 & 587 & 1768 & 84\\
\addlinespace
46 & 4 & 1852 & 1852 & 566 & 1286 & 1161 & 691\\
46 & 4 & 1852 & 1852 & 536 & 1316 & 1809 & 43\\
46 & 4 & 1852 & 1852 & 1502 & 350 & 441 & 1411\\
46 & 4 & 1852 & 1852 & 454 & 1398 & 1820 & 32\\
46 & 4 & 1852 & 1852 & 773 & 1079 & 1455 & 397\\
\addlinespace
47 & 4 & 1852 & 2264 & 655 & 1609 & 1022 & 830\\
47 & 4 & 1852 & 2264 & 1457 & 807 & 1310 & 542\\
47 & 4 & 1852 & 2264 & 1287 & 977 & 530 & 1322\\
47 & 4 & 1852 & 2264 & 100 & 2164 & 176 & 1676\\
47 & 4 & 1852 & 2264 & 107 & 2157 & 1339 & 513\\*
\end{longtable}


==> graphs_export/experiment/trials_table3.tex <==
\begin{longtable}[t]{rrrrrrrr}
\caption{Overview of 240 trials of the altruism task \label{tab:trials_overview}}\\
\toprule
\multicolumn{2}{c}{Game Identifiers} & \multicolumn{2}{c}{Payments} & \multicolumn{4}{c}{Components of Sums (Treatment)} \\
\cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-4} \cmidrule(l{3pt}r{3pt}){5-8}
Game ID & Game Group & Other & Self & Self 1 & Self 2 & Other 1 & Other 2\\
\midrule
\endfirsthead
\caption[]{Overview of 240 trials of the altruism task  \textit{(continued)}}\\
\toprule
\multicolumn{2}{c}{Game Identifiers} & \multicolumn{2}{c}{Payments} & \multicolumn{4}{c}{Components of Sums (Treatment)} \\
\cmidrule(l{3pt}r{3pt}){1-2} \cmidrule(l{3pt}r{3pt}){3-4} \cmidrule(l{3pt}r{3pt}){5-8}
Game ID & Game Group & Other & Self & Self 1 & Self 2 & Other 1 & Other 2\\
\midrule
\endhead

\endfoot
\bottomrule
\endlastfoot
0 & 1 & 655 & 0 & 0 & 0 & 543 & 112\\
0 & 1 & 655 & 0 & 0 & 0 & 629 & 26\\
0 & 1 & 655 & 0 & 0 & 0 & 490 & 165\\
0 & 1 & 655 & 0 & 0 & 0 & 32 & 623\\
0 & 1 & 655 & 0 & 0 & 0 & 540 & 115\\
\addlinespace
1 & 1 & 655 & 34 & 14 & 20 & 638 & 17\\
1 & 1 & 655 & 34 & 23 & 11 & 20 & 635\\
1 & 1 & 655 & 34 & 22 & 12 & 643 & 12\\
1 & 1 & 655 & 34 & 15 & 19 & 14 & 641\\
1 & 1 & 655 & 34 & 22 & 12 & 10 & 645\\
\addlinespace
2 & 1 & 655 & 72 & 24 & 48 & 627 & 28\\
2 & 1 & 655 & 72 & 35 & 37 & 34 & 621\\
2 & 1 & 655 & 72 & 58 & 14 & 26 & 629\\
2 & 1 & 655 & 72 & 61 & 11 & 40 & 615\\
2 & 1 & 655 & 72 & 37 & 35 & 35 & 620\\
\addlinespace
3 & 1 & 655 & 115 & 31 & 84 & 33 & 622\\
3 & 1 & 655 & 115 & 36 & 79 & 621 & 34\\
3 & 1 & 655 & 115 & 39 & 76 & 617 & 38\\
3 & 1 & 655 & 115 & 28 & 87 & 645 & 10\\
3 & 1 & 655 & 115 & 34 & 81 & 585 & 70\\
\addlinespace
4 & 1 & 655 & 163 & 62 & 101 & 11 & 644\\
4 & 1 & 655 & 163 & 12 & 151 & 10 & 645\\
4 & 1 & 655 & 163 & 15 & 148 & 643 & 12\\
4 & 1 & 655 & 163 & 13 & 150 & 643 & 12\\
4 & 1 & 655 & 163 & 140 & 23 & 554 & 101\\
\addlinespace
5 & 1 & 655 & 218 & 167 & 51 & 47 & 608\\
5 & 1 & 655 & 218 & 164 & 54 & 509 & 146\\
5 & 1 & 655 & 218 & 172 & 46 & 622 & 33\\
5 & 1 & 655 & 218 & 81 & 137 & 41 & 614\\
5 & 1 & 655 & 218 & 18 & 200 & 122 & 533\\
\addlinespace
6 & 1 & 655 & 280 & 170 & 110 & 588 & 67\\
6 & 1 & 655 & 280 & 234 & 46 & 60 & 595\\
6 & 1 & 655 & 280 & 90 & 190 & 104 & 551\\
6 & 1 & 655 & 280 & 161 & 119 & 506 & 149\\
6 & 1 & 655 & 280 & 126 & 154 & 15 & 640\\
\addlinespace
7 & 1 & 655 & 352 & 107 & 245 & 557 & 98\\
7 & 1 & 655 & 352 & 161 & 191 & 68 & 587\\
7 & 1 & 655 & 352 & 227 & 125 & 583 & 72\\
7 & 1 & 655 & 352 & 310 & 42 & 645 & 10\\
7 & 1 & 655 & 352 & 170 & 182 & 486 & 169\\
\addlinespace
8 & 1 & 655 & 436 & 68 & 368 & 51 & 604\\
8 & 1 & 655 & 436 & 331 & 105 & 97 & 558\\
8 & 1 & 655 & 436 & 425 & 11 & 485 & 170\\
8 & 1 & 655 & 436 & 326 & 110 & 634 & 21\\
8 & 1 & 655 & 436 & 312 & 124 & 158 & 497\\
\addlinespace
9 & 1 & 655 & 535 & 199 & 336 & 471 & 184\\
9 & 1 & 655 & 535 & 413 & 122 & 71 & 584\\
9 & 1 & 655 & 535 & 398 & 137 & 27 & 628\\
9 & 1 & 655 & 535 & 426 & 109 & 478 & 177\\
9 & 1 & 655 & 535 & 222 & 313 & 443 & 212\\
\addlinespace
10 & 1 & 655 & 655 & 253 & 402 & 79 & 576\\
10 & 1 & 655 & 655 & 277 & 378 & 82 & 573\\
10 & 1 & 655 & 655 & 332 & 323 & 575 & 80\\
10 & 1 & 655 & 655 & 361 & 294 & 565 & 90\\
10 & 1 & 655 & 655 & 156 & 499 & 419 & 236\\
\addlinespace
11 & 1 & 655 & 800 & 740 & 60 & 515 & 140\\
11 & 1 & 655 & 800 & 678 & 122 & 260 & 395\\
11 & 1 & 655 & 800 & 503 & 297 & 635 & 20\\
11 & 1 & 655 & 800 & 311 & 489 & 39 & 616\\
11 & 1 & 655 & 800 & 744 & 56 & 244 & 411\\
\addlinespace
12 & 2 & 926 & 0 & 0 & 0 & 850 & 76\\
12 & 2 & 926 & 0 & 0 & 0 & 836 & 90\\
12 & 2 & 926 & 0 & 0 & 0 & 254 & 672\\
12 & 2 & 926 & 0 & 0 & 0 & 418 & 508\\
12 & 2 & 926 & 0 & 0 & 0 & 391 & 535\\
\addlinespace
13 & 2 & 926 & 48 & 13 & 35 & 10 & 916\\
13 & 2 & 926 & 48 & 11 & 37 & 10 & 916\\
13 & 2 & 926 & 48 & 36 & 12 & 19 & 907\\
13 & 2 & 926 & 48 & 32 & 16 & 26 & 900\\
13 & 2 & 926 & 48 & 30 & 18 & 914 & 12\\
\addlinespace
14 & 2 & 926 & 102 & 84 & 18 & 11 & 915\\
14 & 2 & 926 & 102 & 39 & 63 & 32 & 894\\
14 & 2 & 926 & 102 & 76 & 26 & 909 & 17\\
14 & 2 & 926 & 102 & 35 & 67 & 19 & 907\\
14 & 2 & 926 & 102 & 66 & 36 & 20 & 906\\
\addlinespace
15 & 2 & 926 & 163 & 70 & 93 & 69 & 857\\
15 & 2 & 926 & 163 & 138 & 25 & 28 & 898\\
15 & 2 & 926 & 163 & 111 & 52 & 48 & 878\\
15 & 2 & 926 & 163 & 39 & 124 & 114 & 812\\
15 & 2 & 926 & 163 & 25 & 138 & 17 & 909\\
\addlinespace
16 & 2 & 926 & 231 & 214 & 17 & 16 & 910\\
16 & 2 & 926 & 231 & 62 & 169 & 53 & 873\\
16 & 2 & 926 & 231 & 35 & 196 & 914 & 12\\
16 & 2 & 926 & 231 & 67 & 164 & 864 & 62\\
16 & 2 & 926 & 231 & 161 & 70 & 126 & 800\\
\addlinespace
17 & 2 & 926 & 308 & 90 & 218 & 45 & 881\\
17 & 2 & 926 & 308 & 101 & 207 & 169 & 757\\
17 & 2 & 926 & 308 & 22 & 286 & 905 & 21\\
17 & 2 & 926 & 308 & 84 & 224 & 38 & 888\\
17 & 2 & 926 & 308 & 173 & 135 & 99 & 827\\
\addlinespace
18 & 2 & 926 & 396 & 11 & 385 & 10 & 916\\
18 & 2 & 926 & 396 & 184 & 212 & 733 & 193\\
18 & 2 & 926 & 396 & 74 & 322 & 45 & 881\\
18 & 2 & 926 & 396 & 170 & 226 & 896 & 30\\
18 & 2 & 926 & 396 & 325 & 71 & 187 & 739\\
\addlinespace
19 & 2 & 926 & 498 & 63 & 435 & 51 & 875\\
19 & 2 & 926 & 498 & 264 & 234 & 879 & 47\\
19 & 2 & 926 & 498 & 330 & 168 & 273 & 653\\
19 & 2 & 926 & 498 & 325 & 173 & 779 & 147\\
19 & 2 & 926 & 498 & 366 & 132 & 50 & 876\\
\addlinespace
20 & 2 & 926 & 617 & 486 & 131 & 200 & 726\\
20 & 2 & 926 & 617 & 410 & 207 & 148 & 778\\
20 & 2 & 926 & 617 & 409 & 208 & 775 & 151\\
20 & 2 & 926 & 617 & 416 & 201 & 186 & 740\\
20 & 2 & 926 & 617 & 106 & 511 & 470 & 456\\
\addlinespace
21 & 2 & 926 & 757 & 565 & 192 & 171 & 755\\
21 & 2 & 926 & 757 & 604 & 153 & 106 & 820\\
21 & 2 & 926 & 757 & 480 & 277 & 152 & 774\\
21 & 2 & 926 & 757 & 557 & 200 & 821 & 105\\
21 & 2 & 926 & 757 & 733 & 24 & 470 & 456\\
\addlinespace
22 & 2 & 926 & 926 & 224 & 702 & 647 & 279\\
22 & 2 & 926 & 926 & 79 & 847 & 730 & 196\\
22 & 2 & 926 & 926 & 117 & 809 & 83 & 843\\
22 & 2 & 926 & 926 & 46 & 880 & 727 & 199\\
22 & 2 & 926 & 926 & 370 & 556 & 567 & 359\\
\addlinespace
23 & 2 & 926 & 1132 & 827 & 305 & 711 & 215\\
23 & 2 & 926 & 1132 & 669 & 463 & 146 & 780\\
23 & 2 & 926 & 1132 & 1072 & 60 & 863 & 63\\
23 & 2 & 926 & 1132 & 598 & 534 & 222 & 704\\
23 & 2 & 926 & 1132 & 867 & 265 & 323 & 603\\
\addlinespace
24 & 3 & 1310 & 0 & 0 & 0 & 963 & 347\\
24 & 3 & 1310 & 0 & 0 & 0 & 898 & 412\\
24 & 3 & 1310 & 0 & 0 & 0 & 726 & 584\\
24 & 3 & 1310 & 0 & 0 & 0 & 876 & 434\\
24 & 3 & 1310 & 0 & 0 & 0 & 459 & 851\\
\addlinespace
25 & 3 & 1310 & 68 & 35 & 33 & 1288 & 22\\
25 & 3 & 1310 & 68 & 28 & 40 & 1294 & 16\\
25 & 3 & 1310 & 68 & 31 & 37 & 26 & 1284\\
25 & 3 & 1310 & 68 & 26 & 42 & 10 & 1300\\
25 & 3 & 1310 & 68 & 29 & 39 & 1283 & 27\\
\addlinespace
26 & 3 & 1310 & 145 & 121 & 24 & 1288 & 22\\
26 & 3 & 1310 & 145 & 42 & 103 & 1293 & 17\\
26 & 3 & 1310 & 145 & 79 & 66 & 1286 & 24\\
26 & 3 & 1310 & 145 & 121 & 24 & 1212 & 98\\
26 & 3 & 1310 & 145 & 14 & 131 & 1298 & 12\\
\addlinespace
27 & 3 & 1310 & 231 & 80 & 151 & 1292 & 18\\
27 & 3 & 1310 & 231 & 140 & 91 & 10 & 1300\\
27 & 3 & 1310 & 231 & 34 & 197 & 110 & 1200\\
27 & 3 & 1310 & 231 & 35 & 196 & 28 & 1282\\
27 & 3 & 1310 & 231 & 127 & 104 & 74 & 1236\\
\addlinespace
28 & 3 & 1310 & 327 & 182 & 145 & 1238 & 72\\
28 & 3 & 1310 & 327 & 167 & 160 & 1259 & 51\\
28 & 3 & 1310 & 327 & 62 & 265 & 1257 & 53\\
28 & 3 & 1310 & 327 & 242 & 85 & 1154 & 156\\
28 & 3 & 1310 & 327 & 79 & 248 & 1124 & 186\\
\addlinespace
29 & 3 & 1310 & 436 & 346 & 90 & 1293 & 17\\
29 & 3 & 1310 & 436 & 261 & 175 & 153 & 1157\\
29 & 3 & 1310 & 436 & 112 & 324 & 1233 & 77\\
29 & 3 & 1310 & 436 & 143 & 293 & 215 & 1095\\
29 & 3 & 1310 & 436 & 145 & 291 & 72 & 1238\\
\addlinespace
30 & 3 & 1310 & 561 & 298 & 263 & 1040 & 270\\
30 & 3 & 1310 & 561 & 550 & 11 & 10 & 1300\\
30 & 3 & 1310 & 561 & 202 & 359 & 1254 & 56\\
30 & 3 & 1310 & 561 & 515 & 46 & 934 & 376\\
30 & 3 & 1310 & 561 & 470 & 91 & 884 & 426\\
\addlinespace
31 & 3 & 1310 & 705 & 655 & 50 & 1273 & 37\\
31 & 3 & 1310 & 705 & 442 & 263 & 1161 & 149\\
31 & 3 & 1310 & 705 & 665 & 40 & 278 & 1032\\
31 & 3 & 1310 & 705 & 627 & 78 & 21 & 1289\\
31 & 3 & 1310 & 705 & 597 & 108 & 10 & 1300\\
\addlinespace
32 & 3 & 1310 & 873 & 849 & 24 & 521 & 789\\
32 & 3 & 1310 & 873 & 704 & 169 & 1292 & 18\\
32 & 3 & 1310 & 873 & 758 & 115 & 1271 & 39\\
32 & 3 & 1310 & 873 & 395 & 478 & 62 & 1248\\
32 & 3 & 1310 & 873 & 832 & 41 & 783 & 527\\
\addlinespace
33 & 3 & 1310 & 1071 & 512 & 559 & 416 & 894\\
33 & 3 & 1310 & 1071 & 246 & 825 & 217 & 1093\\
33 & 3 & 1310 & 1071 & 942 & 129 & 72 & 1238\\
33 & 3 & 1310 & 1071 & 493 & 578 & 1262 & 48\\
33 & 3 & 1310 & 1071 & 718 & 353 & 656 & 654\\
\addlinespace
34 & 3 & 1310 & 1310 & 108 & 1202 & 814 & 496\\
34 & 3 & 1310 & 1310 & 63 & 1247 & 1149 & 161\\
34 & 3 & 1310 & 1310 & 750 & 560 & 219 & 1091\\
34 & 3 & 1310 & 1310 & 944 & 366 & 235 & 1075\\
34 & 3 & 1310 & 1310 & 304 & 1006 & 254 & 1056\\
\addlinespace
35 & 3 & 1310 & 1601 & 1045 & 556 & 575 & 735\\
35 & 3 & 1310 & 1601 & 1005 & 596 & 637 & 673\\
35 & 3 & 1310 & 1601 & 1465 & 136 & 800 & 510\\
35 & 3 & 1310 & 1601 & 1459 & 142 & 667 & 643\\
35 & 3 & 1310 & 1601 & 1134 & 467 & 587 & 723\\
\addlinespace
36 & 4 & 1852 & 0 & 0 & 0 & 622 & 1230\\
36 & 4 & 1852 & 0 & 0 & 0 & 1453 & 399\\
36 & 4 & 1852 & 0 & 0 & 0 & 1022 & 830\\
36 & 4 & 1852 & 0 & 0 & 0 & 1110 & 742\\
36 & 4 & 1852 & 0 & 0 & 0 & 734 & 1118\\
\addlinespace
37 & 4 & 1852 & 97 & 85 & 12 & 10 & 1842\\
37 & 4 & 1852 & 97 & 34 & 63 & 27 & 1825\\
37 & 4 & 1852 & 97 & 43 & 54 & 41 & 1811\\
37 & 4 & 1852 & 97 & 27 & 70 & 1828 & 24\\
37 & 4 & 1852 & 97 & 37 & 60 & 54 & 1798\\
\addlinespace
38 & 4 & 1852 & 205 & 54 & 151 & 1740 & 112\\
38 & 4 & 1852 & 205 & 91 & 114 & 1777 & 75\\
38 & 4 & 1852 & 205 & 57 & 148 & 1818 & 34\\
38 & 4 & 1852 & 205 & 83 & 122 & 1785 & 67\\
38 & 4 & 1852 & 205 & 122 & 83 & 113 & 1739\\
\addlinespace
39 & 4 & 1852 & 326 & 216 & 110 & 24 & 1828\\
39 & 4 & 1852 & 326 & 109 & 217 & 198 & 1654\\
39 & 4 & 1852 & 326 & 45 & 281 & 198 & 1654\\
39 & 4 & 1852 & 326 & 64 & 262 & 239 & 1613\\
39 & 4 & 1852 & 326 & 222 & 104 & 81 & 1771\\
\addlinespace
40 & 4 & 1852 & 463 & 74 & 389 & 188 & 1664\\
40 & 4 & 1852 & 463 & 293 & 170 & 77 & 1775\\
40 & 4 & 1852 & 463 & 385 & 78 & 1821 & 31\\
40 & 4 & 1852 & 463 & 150 & 313 & 1706 & 146\\
40 & 4 & 1852 & 463 & 259 & 204 & 171 & 1681\\
\addlinespace
41 & 4 & 1852 & 617 & 367 & 250 & 61 & 1791\\
41 & 4 & 1852 & 617 & 331 & 286 & 1708 & 144\\
41 & 4 & 1852 & 617 & 85 & 532 & 1817 & 35\\
41 & 4 & 1852 & 617 & 414 & 203 & 1838 & 14\\
41 & 4 & 1852 & 617 & 302 & 315 & 277 & 1575\\
\addlinespace
42 & 4 & 1852 & 793 & 50 & 743 & 1358 & 494\\
42 & 4 & 1852 & 793 & 649 & 144 & 42 & 1810\\
42 & 4 & 1852 & 793 & 698 & 95 & 66 & 1786\\
42 & 4 & 1852 & 793 & 431 & 362 & 348 & 1504\\
42 & 4 & 1852 & 793 & 245 & 548 & 142 & 1710\\
\addlinespace
43 & 4 & 1852 & 997 & 239 & 758 & 1188 & 664\\
43 & 4 & 1852 & 997 & 964 & 33 & 960 & 892\\
43 & 4 & 1852 & 997 & 768 & 229 & 1774 & 78\\
43 & 4 & 1852 & 997 & 374 & 623 & 330 & 1522\\
43 & 4 & 1852 & 997 & 772 & 225 & 1442 & 410\\
\addlinespace
44 & 4 & 1852 & 1235 & 1069 & 166 & 1318 & 534\\
44 & 4 & 1852 & 1235 & 1055 & 180 & 759 & 1093\\
44 & 4 & 1852 & 1235 & 103 & 1132 & 1781 & 71\\
44 & 4 & 1852 & 1235 & 715 & 520 & 1516 & 336\\
44 & 4 & 1852 & 1235 & 307 & 928 & 1636 & 216\\
\addlinespace
45 & 4 & 1852 & 1515 & 1276 & 239 & 1119 & 733\\
45 & 4 & 1852 & 1515 & 1276 & 239 & 118 & 1734\\
45 & 4 & 1852 & 1515 & 1237 & 278 & 921 & 931\\
45 & 4 & 1852 & 1515 & 1165 & 350 & 749 & 1103\\
45 & 4 & 1852 & 1515 & 928 & 587 & 1768 & 84\\
\addlinespace
46 & 4 & 1852 & 1852 & 566 & 1286 & 1161 & 691\\
46 & 4 & 1852 & 1852 & 536 & 1316 & 1809 & 43\\
46 & 4 & 1852 & 1852 & 1502 & 350 & 441 & 1411\\
46 & 4 & 1852 & 1852 & 454 & 1398 & 1820 & 32\\
46 & 4 & 1852 & 1852 & 773 & 1079 & 1455 & 397\\
\addlinespace
47 & 4 & 1852 & 2264 & 655 & 1609 & 1022 & 830\\
47 & 4 & 1852 & 2264 & 1457 & 807 & 1310 & 542\\
47 & 4 & 1852 & 2264 & 1287 & 977 & 530 & 1322\\
47 & 4 & 1852 & 2264 & 100 & 2164 & 176 & 1676\\
47 & 4 & 1852 & 2264 & 107 & 2157 & 1339 & 513\\*
\end{longtable}


==> graphs_export/meta_cognition/meta_cognition_correlations.tex <==

\centering\begingroup\fontsize{10}{12}\selectfont

\begin{tabular}[b]{>{\raggedright\arraybackslash}p{5cm}>{\raggedright\arraybackslash}p{1.5cm}>{\raggedright\arraybackslash}p{1.5cm}>{\raggedright\arraybackslash}p{1.5cm}>{\raggedright\arraybackslash}p{1.5cm}>{\raggedright\arraybackslash}p{1.5cm}>{\raggedright\arraybackslash}p{1.5cm}}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Altruism (Avg.)} & \multicolumn{3}{c}{Number Comparison (Avg.)} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
  & Choice $Self$ & Std. Deviation  & RT & Choice Correct & Std. Deviation & RT \\
\midrule
\textit{Altruism:} &  &  &  &  &  & \\
Negative Confidence & 0.088 & 0.317*** & 0.080 & -0.127* & 0.109 & 0.048\\
Avg. Attention & -0.215*** & -0.045 & 0.115* & 0.094 & -0.078 & -0.066\\
Precision & -0.195*** & -0.114 & 0.126* & 0.006 & -0.005 & -0.040\\
 &  &  &  &  &  & \\

\textit{Number Comparison:} &  &  &  &  &  & \\
$|\Delta$ Belief Correct$|$ & -0.057 & 0.257*** & 0.198*** & -0.365*** & 0.392*** & 0.433***\\
Belief Correct Confidence & 0.043 & -0.161** & -0.203*** & 0.309*** & -0.285*** & -0.365***\\
$|\Delta$ Belief Time Spent$|$ & 0.074 & 0.107 & 0.125* & -0.077 & 0.040 & 0.209***\\
Belief Time Spent Confidence & 0.033 & 0.003 & -0.121* & 0.025 & -0.031 & -0.151**\\

Precision & 0.020 & -0.017 & -0.113 & 0.254*** & -0.256*** & -0.150*\\
Avg. Attention & 0.008 & -0.131* & -0.093 & 0.223*** & -0.231*** & -0.058\\
\bottomrule
\end{tabular}
\endgroup{}



==> graphs_export/meta_cognition/meta_cognition_treatment.tex <==

\centering\begingroup\fontsize{10}{12}\selectfont

\begin{tabular}[b]{>{\raggedright\arraybackslash}p{5cm}>{\raggedright\arraybackslash}p{1.5cm}>{\raggedright\arraybackslash}p{1.5cm}>{\raggedright\arraybackslash}p{2cm}}
\toprule
  & Baseline (avg.) & Treatment (avg.) & $p$\\
\midrule
\textit{Altruism:} &  &  & \\
Negative Confidence & 0.304 & 0.318 & 0.643\\
Avg. Attention & 0.731 & 0.698 & 0.127\\
Precision & 0.364 & 0.382 & 0.573\\
 &  &  & \\

\textit{Number Comparison:} &  &  & \\
$|\Delta$ Belief Correct$|$ & 0.084 & 0.163 & $<$0.001***\\
Belief Correct Confidence & 0.785 & 0.651 & $<$0.001***\\
$|\Delta$ Belief Time Spent$|$ & 0.674 & 0.976 & 0.01***\\
Belief Time Spent Confidence & 0.638 & 0.593 & 0.093*\\

Precision & 0.568 & 0.447 & $<$0.001***\\
Avg. Attention & 0.761 & 0.705 & 0.007***\\
\bottomrule
\end{tabular}
\endgroup{}



==> graphs_export/results/main_regression_learning.tex <==
\begin{table}[H]

\caption{Main Treatment Effect Regression Learning: Linear Probability Model \label{tab:reg_main}}
\centering
\fontsize{10}{12}\selectfont
\begin{tabular}[t]{lcccc}
\toprule
  & (1) & (2) & (3) & (4)\\
\midrule
Treatment Group & -0.014** & -0.014 & 0.009 & -0.014\\
 & (0.006) & (0.023) & (0.030) & (0.024)\\
Ratio self/other & 0.867*** & 0.867*** & 0.900*** & 0.867***\\
 & (0.004) & (0.013) & (0.018) & (0.003)\\
Treatment Group * Ratio &  &  & -0.067** & \\
 &  &  & (0.026) & \\
Intercept & 0.052*** & 0.052*** & 0.032 & 0.052***\\
 & (0.005) & (0.019) & (0.021) & (0.017)\\
\midrule
Random Effects & No & No & No & Yes\\
Clustered Standard Errors & No & Yes & Yes & Yes\\
Num.Obs. & 72000 & 72000 & 72000 & 72000\\
Unique Obs & 300 & 300 & 300 & 300\\
R2 & 0.430 & 0.430 & 0.431 & 0.517\\
\bottomrule
\multicolumn{5}{l}{\rule{0pt}{1em}* p $<$ 0.1, ** p $<$ 0.05, *** p $<$ 0.01}\\
\end{tabular}
\end{table}


==> graphs_export/results/meta_cognition_regression.tex <==
\begin{table}

\caption{Main Treatment Effect Regression: Linear Probability Model \label{tab:meta_cognition}}
\centering
\fontsize{10}{12}\selectfont
\begin{tabular}[t]{lcccc}
\toprule
  & (1) & (2) & (3) & (4)\\
\midrule
Intercept & -0.490* & -1.613*** & -0.012 & -1.243***\\
 & (0.256) & (0.186) & (0.259) & (0.121)\\
Treatment Group & -0.115 & -0.093 & -0.135 & -0.093\\
 & (0.097) & (0.098) & (0.098) & (0.098)\\
Ratio self/other & 2.212*** & 3.362*** & 1.268*** & 2.914***\\
 & (0.422) & (0.292) & (0.391) & (0.195)\\
Meta Cognition Index & -1.779*** &  &  & \\
 & (0.454) &  &  & \\
Ratio * Meta Cognition Index & 1.528** &  &  & \\
 & (0.685) &  &  & \\
Confidence &  & 0.133 &  & \\
 &  & (0.271) &  & \\
Ratio * Confidence &  & -0.423 &  & \\
 &  & (0.405) &  & \\
Mean Attention &  &  & -2.182*** & \\
 &  &  & (0.345) & \\
Ratio * Mean Attention &  &  & 2.675*** & \\
 &  &  & (0.531) & \\
Precision &  &  &  & -0.799**\\
 &  &  &  & (0.328)\\
Ratio * Precision &  &  &  & 0.496\\
 &  &  &  & (0.438)\\
\midrule
Random Effects & Yes & Yes & Yes & Yes\\
Clustered Standard Errors & Yes & Yes & Yes & Yes\\
Unique Obs & 300 & 300 & 300 & 300\\
Num.Obs. & 72000 & 72000 & 72000 & 72000\\
\bottomrule
\multicolumn{5}{l}{\rule{0pt}{1em}* p $<$ 0.1, ** p $<$ 0.05, *** p $<$ 0.01}\\
\end{tabular}
\end{table}


==> graphs_export/results/symmetric_treatment.tex <==

\centering\begingroup\fontsize{10}{12}\selectfont

\begin{tabular}[b]{>{\raggedright\arraybackslash}p{5cm}>{\raggedleft\arraybackslash}p{1.5cm}>{\raggedleft\arraybackslash}p{1.5cm}>{\raggedright\arraybackslash}p{2cm}}
\toprule
Region & Baseline (avg.) & Treatment (avg.) & $p$\\
\midrule
0.43  $\le \frac{self}{other} \le$ 0.54 & 0.518 & 0.455 & $<$0.001***\\
0.33  $\le \frac{self}{other} \le$ 0.67 & 0.524 & 0.469 & $<$0.001***\\
0.25  $\le \frac{self}{other} \le$ 0.82 & 0.525 & 0.481 & $<$0.001***\\
0.18  $\le \frac{self}{other} \le$ 1 & 0.533 & 0.497 & $<$0.001***\\
0.11  $\le \frac{self}{other} \le$ 1.22 & 0.535 & 0.505 & $<$0.001***\\
\bottomrule
\end{tabular}
\endgroup{}



==> graphs_export/structural_estimation/combined_parameters.tex <==

\begin{tabular}[b]{llllll}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
\textit{Individual Parameters (avg.):} &  &  &  &  & \\
Altr. Preference $\beta_i$ & 0.342 & 0.341 & 0.272 & 0.415 & 1\\
Noise $\nu_{i}$ & 0.336 & 0.323 & 0.186 & 0.515 & 1\\
Prior Std. Outcomes $\sigma^{\hat{r}}_i$ & 1.019 & 0.809 & 0.173 & 2.34 & 1.001\\
Prior Std. Preference $\sigma^{\hat{b}}_i$ & 0.772 & 0.591 & 0.084 & 1.885 & 1.001\\
\addlinespace
Prior Mean Outcomes $\mu^{\hat{r}}_i$ & 1.023 & 0.862 & 0.186 & 2.19 & 1\\
Prior Mean Altr. Preference $\mu^{\hat{b}}_i$ & 0.797 & 0.585 & 0.071 & 2.017 & 1.002\\
Weight on Payments $\alpha_{i}$ & 0.812 & 0.822 & 0.648 & 0.955 & 1\\
Prior Threshold $\delta_{i}$ & 0.852 & 0.846 & 0.559 & 1.139 & 1.001\\
Weight on Preferences $\gamma_{i}$ & 0.717 & 0.745 & 0.372 & 0.981 & 1.001\\
\addlinespace
 &  &  &  &  & \\
\textit{Additional Parameter Information (avg.):} &  &  &  &  & \\
Noise Baseline $\nu_{iB}$ & 0.3 & 0.289 & 0.171 & 0.453 & 1\\
Noise Treatment $\nu_{iT}$ & 0.372 & 0.357 & 0.2 & 0.577 & 1\\
$\sigma^{\hat{r}}_i - \sigma^{\hat{b}}_i$ & 0.246 & 0.211 & -1.87 & 2.452 & 1.003\\
\addlinespace
$\mu^{\hat{r}}_i - \mu^{\hat{b}}_i$ & 0.226 & 0.258 & -1.577 & 2.033 & 1\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/combined_parameters_arithmetics.tex <==

\begin{tabular}[b]{llllll}
\toprule
  & mean & sd & hdi 3\% & hdi 97\% & $\hat{R}$\\
\midrule
\textit{Hyper-Parameters:} &  &  &  &  & \\
Mean $\nu$ Baseline $\mu_{B}^{\nu'}$ & -1.791 & 0.052 & -1.89 & -1.693 & 1\\
Mean $\nu$ Treatment $\mu_{T}^{\nu'}$ & -1.387 & 0.036 & -1.454 & -1.32 & 1\\
Diff. means $\nu$ $\mu_{T}^{\nu'} - \mu_{B}^{\nu'}$ & 0.404 & 0.063 & 0.29 & 0.525 & 1\\
Std. $\nu$ Baseline $\sigma_{B}^{\nu'}$ & 0.619 & 0.042 & 0.542 & 0.698 & 1\\
\addlinespace
Std. $\nu$ Treatment $\sigma_{T}^{\nu'}$ & 0.403 & 0.029 & 0.349 & 0.459 & 1\\
 &  &  &  &  & \\
\textit{Individual Parameters (avg.):} &  &  &  &  & \\
Noise Baseline $\nu_{iB}^{'}$ & 0.197 & 0.029 & 0.145 & 0.252 & 1\\
Noise Treatment $\nu_{iT}^{'}$ & 0.27 & 0.038 & 0.202 & 0.342 & 1\\
\addlinespace
Prior Mean Outcomes $\mu^{\hat{r}'}_i$ & 0.87 & 0.289 & 0.356 & 1.399 & 1\\
Prior Std. Outcomes $\sigma^{\hat{r}'}_i$ & 2.084 & 2.229 & 0.181 & 5.297 & 1\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/combined_parameters_number.tex <==

\begin{tabular}[b]{llllll}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
\textit{Individual Parameters (avg.):} &  &  &  &  & \\
Noise $\nu_{i}'$ & 0.233 & 0.23 & 0.172 & 0.301 & 1\\
Prior Std. Outcomes $\sigma^{\hat{r}'}_{i}$ & 0.785 & 0.762 & 0.455 & 1.153 & 1.014\\
Prior Mean Outcomes $\mu^{\hat{r}'}_{i}$ & 0.518 & 0.46 & 0.157 & 0.994 & 1.002\\
Weight on Payments $\alpha_{i}'$ & 0.905 & 0.911 & 0.827 & 0.969 & 1.011\\
\addlinespace
Prior Threshold $\delta_{i}'$ & 1.103 & 1.098 & 1.021 & 1.193 & 1.003\\
 &  &  &  &  & \\
\textit{Additional Parameter Information (avg.):} &  &  &  &  & \\
Noise Baseline $\nu_{iB'}$ & 0.197 & 0.194 & 0.144 & 0.255 & 1\\
Noise Treatment $\nu_{iT'}$ & 0.27 & 0.266 & 0.199 & 0.347 & 1\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/combined_parameters_prior.tex <==

\begin{tabular}[b]{lllll}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\%\\
\midrule
\textit{Individual Parameters (avg.):} &  &  &  & \\
Altr. Preference $\beta_i$ & 0.287 & 0.271 & 0.036 & 0.543\\
Noise $\nu_{i}$ & 1.074 & 0.985 & 0.348 & 1.916\\
Prior Std. Outcomes $\sigma^{\hat{r}}_i$ & 1.06 & 0.991 & 0.418 & 1.776\\
Prior Std. Preference $\sigma^{\hat{b}}_i$ & 1.083 & 0.995 & 0.381 & 1.912\\
\addlinespace
Prior Mean Outcomes $\mu^{\hat{r}}_i$ & 0.822 & 0.765 & 0.31 & 1.408\\
Prior Mean Altr. Preference $\mu^{\hat{b}}_i$ & 0.838 & 0.781 & 0.32 & 1.437\\
 &  &  &  & \\
\textit{Additional Parameter Information (avg.):} &  &  &  & \\
$\sigma^{\hat{r}}_i - \sigma^{\hat{b}}_i$ & -0.022 & -0.016 & -1.184 & 1.071\\
\addlinespace
$\mu^{\hat{r}}_i - \mu^{\hat{b}}_i$ & -0.016 & -0.006 & -0.86 & 0.858\\
$\mu_{T}^{\nu'} - \mu_{B}^{\nu'}$ & -0.012 & -0.006 & -0.493 & 0.457\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/correlation_estimates_behavior.tex <==
\begin{tabular}[b]{>{\raggedright\arraybackslash}p{4cm}>{\raggedright\arraybackslash}p{3cm}>{\raggedright\arraybackslash}p{3cm}}
\toprule
  & Altruism Noise $\nu$ & Altr. Preference $\beta$\\
\midrule
\textit{Cognition-related:} &  & \\
No. Correct CRT & -0.296*** & 0.180**\\
Berlin Numeracy Test & -0.273*** & 0.188**\\
Avg. Need for Cognition & -0.157** & 0.145*\\
Avg. Deliberation & 0.140* & -0.145*\\
\addlinespace
Avg. Intuition & 0.107 & -0.103\\
 &  & \\
\textit{Altruism-related:} &  & \\
Dictator Game Other & -0.317*** & 0.475***\\
GPS Value Gift & -0.090 & 0.132*\\
\addlinespace
GPS Donation & -0.029 & 0.128*\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/main_parameters.tex <==

\begin{tabular}[b]{lrrrrr}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
Altr. Preference $\beta_i$ & 0.342 & 0.341 & 0.272 & 0.415 & 1.000\\
Noise $\nu_{i}$ & 0.336 & 0.323 & 0.186 & 0.515 & 1.000\\
Prior Std. Outcomes $\sigma^{\hat{r}}_i$ & 1.019 & 0.809 & 0.173 & 2.340 & 1.001\\
Prior Std. Preference $\sigma^{\hat{b}}_i$ & 0.772 & 0.591 & 0.084 & 1.885 & 1.001\\
Prior Mean Outcomes $\mu^{\hat{r}}_i$ & 1.023 & 0.862 & 0.186 & 2.190 & 1.000\\
\addlinespace
Prior Mean Altr. Preference $\mu^{\hat{b}}_i$ & 0.797 & 0.585 & 0.071 & 2.017 & 1.002\\
Weight on Payments $\alpha_{i}$ & 0.812 & 0.822 & 0.648 & 0.955 & 1.000\\
Prior Threshold $\delta_{i}$ & 0.852 & 0.846 & 0.559 & 1.139 & 1.001\\
Weight on Preferences $\gamma_{i}$ & 0.717 & 0.745 & 0.372 & 0.981 & 1.001\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/main_parameters_arithmetics.tex <==

\begin{tabular}[b]{lrrrrr}
\toprule
  & mean & sd & hdi 3\% & hdi 97\% & $\hat{R}$\\
\midrule
Noise Baseline $\nu_{iB}^{'}$ & 0.197 & 0.029 & 0.145 & 0.252 & 1\\
Noise Treatment $\nu_{iT}^{'}$ & 0.270 & 0.038 & 0.202 & 0.342 & 1\\
Prior Mean Outcomes $\mu^{\hat{r}'}_i$ & 0.870 & 0.289 & 0.356 & 1.399 & 1\\
Prior Std. Outcomes $\sigma^{\hat{r}'}_i$ & 2.084 & 2.229 & 0.181 & 5.297 & 1\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/main_parameters_info.tex <==

\begin{tabular}[b]{lrrrrr}
\toprule
  & median & mean & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
Noise Baseline $\nu_{iB}$ & 0.289 & 0.300 & 0.171 & 0.453 & 1.000\\
Noise Treatment $\nu_{iT}$ & 0.357 & 0.372 & 0.200 & 0.577 & 1.000\\
$\sigma^{\hat{r}}_i - \sigma^{\hat{b}}_i$ & 0.211 & 0.246 & -1.870 & 2.452 & 1.003\\
$\mu^{\hat{r}}_i - \mu^{\hat{b}}_i$ & 0.258 & 0.226 & -1.577 & 2.033 & 1.000\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/main_parameters_info_prior.tex <==

\begin{tabular}[b]{lrrrr}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\%\\
\midrule
$\mu^{\nu_{\frac{\beta}{1-\beta}}}_B - \mu^{\nu_{\frac{\beta}{1-\beta}}}_T$ & 0.001 & 0.003 & -0.507 & 0.473\\
$\mu^{\nu_{\frac{\text{self}}{\text{other}}}}_B - \mu^{\nu_{\frac{\text{self}}{\text{other}}}}_T$ & -0.007 & -0.005 & -0.477 & 0.429\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/main_parameters_population.tex <==

\begin{tabular}[b]{lrrrrr}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
$\mu_{T}^{\nu} - \mu_{B}^{\nu}$ & 0.198 & 0.198 & 0.074 & 0.332 & 1.00\\
$\mu^{^{\nu}}$ & -1.402 & -1.403 & -1.537 & -1.268 & 1.00\\
$\mu^{\mu^{^{\hat{r}}}}$ & -0.152 & -0.156 & -0.578 & 0.306 & 1.01\\
$\mu^{\sigma^{^{\hat{b}}}}$ & -0.525 & -0.536 & -0.937 & -0.074 & 1.01\\
$\mu^{\sigma^{^{\hat{r}}}}$ & -0.193 & -0.201 & -0.617 & 0.263 & 1.01\\
\addlinespace
$\mu^{\mu^{^{\hat{b}}}}$ & -0.634 & -0.644 & -1.092 & -0.158 & 1.01\\
$\mu^{^{\frac{\beta}{1-\beta}}}$ & -0.682 & -0.681 & -0.840 & -0.520 & 1.01\\
$\sigma^{^{\nu}}$ & 0.477 & 0.474 & 0.352 & 0.600 & 1.00\\
$\sigma^{^{\frac{\beta}{1-\beta}}}$ & 0.115 & 0.113 & 0.058 & 0.177 & 1.01\\
$\sigma^{\sigma^{^{\hat{b}}}}$ & 0.443 & 0.392 & 0.042 & 0.966 & 1.01\\
\addlinespace
$\sigma^{\sigma^{^{\hat{r}}}}$ & 0.313 & 0.264 & 0.002 & 0.754 & 1.01\\
$\sigma^{\mu^{^{\hat{b}}}}$ & 0.709 & 0.668 & 0.068 & 1.387 & 1.01\\
$\sigma^{\mu^{^{\hat{r}}}}$ & 0.261 & 0.186 & 0.001 & 0.765 & 1.03\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/main_parameters_population_number.tex <==

\begin{tabular}[b]{lrrrrr}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
$\mu^{\mu^{^{\nu}}} & -1.739 & -1.739 & -1.832 & -1.645 & 1.00\\
$\sigma^{\mu^{^{\hat{r}}}}$ & -0.822 & -0.817 & -0.962 & -0.695 & 1.00\\
$\sigma^{\mu^{^{\hat{r}}}}$ & -0.269 & -0.260 & -0.583 & 0.021 & 1.03\\
$\mu_{T}^{\nu} - \mu_{B}^{\nu}$ & 0.348 & 0.349 & 0.200 & 0.484 & 1.00\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/main_parameters_prior.tex <==

\begin{tabular}[b]{lrrrr}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\%\\
\midrule
Altr. Preference $\beta_i$ & 0.287 & 0.271 & 0.036 & 0.543\\
Noise $\nu_{i}$ & 1.074 & 0.985 & 0.348 & 1.916\\
Prior Std. Outcomes $\sigma^{\hat{r}}_i$ & 1.060 & 0.991 & 0.418 & 1.776\\
Prior Std. Preference $\sigma^{\hat{b}}_i$ & 1.083 & 0.995 & 0.381 & 1.912\\
Prior Mean Outcomes $\mu^{\hat{r}}_i$ & 0.822 & 0.765 & 0.310 & 1.408\\
\addlinespace
Prior Mean Altr. Preference $\mu^{\hat{b}}_i$ & 0.838 & 0.781 & 0.320 & 1.437\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/main_parameters_transformed.tex <==

\begin{tabular}[b]{lllllll}
\toprule
  & mean & median & sd & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
\textit{Base Parameters:} &  &  &  &  &  & \\
Altr. Preference $\beta$ & 0.316 & 0.316 & 0.008 & 0.3 & 0.332 & 1\\
Prior Mean Outcomes $\mu^{\hat{r}}$ & 1.049 & 1.005 & 0.304 & 0.533 & 1.652 & 1.01\\
\textit{Group Specific:} &  &  &  &  &  & \\
Noise Baseline $\nu_{B}$ & 0.277 & 0.276 & 0.024 & 0.232 & 0.326 & 1\\
\addlinespace
Noise Treatment $\nu_{T}$ & 0.338 & 0.337 & 0.031 & 0.281 & 0.401 & 1.01\\
Weight on Payments Baseline $\alpha_B$ & 0.902 & 0.906 & 0.042 & 0.819 & 0.979 & 1.01\\
Weight on Payments Treatment $\alpha_T$ & 0.863 & 0.867 & 0.056 & 0.753 & 0.966 & 1.01\\
Weight on Preferences Baseline $\gamma_B$ & 0.837 & 0.848 & 0.084 & 0.671 & 0.982 & 1.01\\
Weight on Preferences Treatment $\gamma_T$ & 0.779 & 0.788 & 0.106 & 0.575 & 0.971 & 1.01\\
\addlinespace
Prior Threshold Baseline $\delta_B$ & 0.958 & 0.96 & 0.08 & 0.79 & 1.112 & 1.01\\
Prior Threshold Treatment $\delta_T$ & 0.946 & 0.945 & 0.107 & 0.73 & 1.152 & 1\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/main_parameters_transformed_commonnoise.tex <==

\begin{tabular}[b]{lllllll}
\toprule
  & mean & median & sd & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
\textit{Base Parameters:} &  &  &  &  &  & \\
Altr. Preference $\beta$ & 0.297 & 0.297 & 0.014 & 0.269 & 0.324 & 1.01\\
Prior Std. Outcomes $\sigma^{\hat{r}}$ & 0.154 & 0.152 & 0.017 & 0.121 & 0.187 & 1.02\\
Prior Mean Outcomes $\mu^{\hat{r}}$ & 0.497 & 0.497 & 0.001 & 0.494 & 0.499 & 1.01\\
Prior Std. Preference $\sigma^{\hat{b}}$ & 0.273 & 0.263 & 0.061 & 0.173 & 0.398 & 1.01\\
Prior Mean Altr. Preference $\mu^{\hat{b}}$ & 0.512 & 0.511 & 0.027 & 0.462 & 0.567 & 1.01\\
\addlinespace
\textit{Group Specific:} &  &  &  &  &  & \\
Noise Baseline $\nu_{B}$ & 0.277 & 0.276 & 0.024 & 0.232 & 0.326 & 1\\
Noise Treatment $\nu_{T}$ & 0.338 & 0.337 & 0.031 & 0.281 & 0.401 & 1.01\\
Weight on Payments Baseline $\alpha_B$ & 0.902 & 0.906 & 0.042 & 0.819 & 0.979 & 1.01\\
Weight on Payments Treatment $\alpha_T$ & 0.863 & 0.867 & 0.056 & 0.753 & 0.966 & 1.01\\
Weight on Preferences Baseline $\gamma_B$ & 0.837 & 0.848 & 0.084 & 0.671 & 0.982 & 1.01\\
Weight on Preferences Treatment $\gamma_T$ & 0.779 & 0.788 & 0.106 & 0.575 & 0.971 & 1.01\\
Prior Treshold Baseline $\delta_B$ & 0.958 & 0.96 & 0.08 & 0.79 & 1.112 & 1.01\\
Prior Treshold Treatment $\delta_T$ & 0.946 & 0.945 & 0.107 & 0.73 & 1.152 & 1\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/main_parameters_transformed_separatenoise.tex <==

\begin{tabular}[b]{lllllll}
\toprule
  & mean & median & sd & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
\textit{Base Parameters:} &  &  &  &  &  & \\
Altr. Preference $\beta$ & 0.269 & 0.265 & 0.044 & 0.19 & 0.361 & 1.01\\
Prior Std. Outcomes $\sigma^{\hat{r}}$ & 0.527 & 0.515 & 0.091 & 0.368 & 0.708 & 1.06\\
Prior Mean Outcomes $\mu^{\hat{r}}$ & 0.466 & 0.468 & 0.017 & 0.429 & 0.496 & 1.02\\
Prior Std. Preference $\sigma^{\hat{b}}$ & 0.755 & 0.741 & 0.102 & 0.578 & 0.962 & 1.03\\
Prior Mean Altr. Preference $\mu^{\hat{b}}$ & 0.586 & 0.583 & 0.044 & 0.509 & 0.679 & 1.01\\
\addlinespace
\textit{Group Specific:} &  &  &  &  &  & \\
Noise Altruism Baseline $\nu_{\frac{\beta}{1-\beta},B}$ & 1.138 & 1.103 & 0.248 & 0.714 & 1.636 & 1\\
Noise Altruism Treatment $\nu_{\frac{\beta}{1-\beta},T}$ & 1.381 & 1.334 & 0.339 & 0.779 & 2.029 & 1\\
Noise Numbers Baseline $\nu_{\frac{self}{other},B}$ & 0.178 & 0.178 & 0.008 & 0.163 & 0.194 & 1\\
Noise Numbers Baseline $\nu_{\frac{self}{other},B}$ & 0.247 & 0.247 & 0.011 & 0.226 & 0.268 & 1\\
Weight on Payments Baseline $\alpha_B$ & 0.89 & 0.894 & 0.035 & 0.824 & 0.951 & 1.06\\
Weight on Payments Treatment $\alpha_T$ & 0.81 & 0.813 & 0.051 & 0.714 & 0.903 & 1.06\\
Weight on Preferences Baseline $\gamma_B$ & 0.32 & 0.311 & 0.104 & 0.136 & 0.53 & 1\\
Weight on Preferences Treatment $\gamma_T$ & 0.25 & 0.237 & 0.098 & 0.08 & 0.443 & 1.01\\
Prior Threshold Numbers Baseline $\delta_{\frac{self}{other},B}$ & 1.087 & 1.085 & 0.027 & 1.04 & 1.14 & 1.06\\
Prior Threshold Altruism Baseline $\delta_{\frac{\beta}{1-\beta},B}$ & 0.728 & 0.723 & 0.062 & 0.616 & 0.854 & 1.01\\
Prior Threshold Numbers Treatment $\delta_{\frac{self}{other},T}$ & 1.156 & 1.153 & 0.042 & 1.078 & 1.236 & 1.05\\
Prior Threshold Altruism Treatment $\delta_{\frac{\beta}{1-\beta},T}$ & 0.774 & 0.768 & 0.067 & 0.653 & 0.906 & 1.01\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/number_parameters.tex <==

\begin{tabular}[b]{lrrrrr}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
Noise $\nu_{i}'$ & 0.233 & 0.230 & 0.172 & 0.301 & 1.000\\
Prior Std. Outcomes $\sigma^{\hat{r}}_{i}'$ & 0.785 & 0.762 & 0.455 & 1.153 & 1.014\\
Prior Mean Outcomes $\mu^{\hat{r}}_{i}'$ & 0.518 & 0.460 & 0.157 & 0.994 & 1.002\\
Weight on Payments$\alpha_{i}'$ & 0.905 & 0.911 & 0.827 & 0.969 & 1.011\\
Prior Threshold $\delta_{i}'$ & 1.103 & 1.098 & 1.021 & 1.193 & 1.003\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/number_parameters_info.tex <==

\begin{tabular}[b]{lrrrrr}
\toprule
  & median & mean & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
Noise Baseline $\nu_{iB'}$ & 0.194 & 0.197 & 0.144 & 0.255 & 1\\
Noise Treatment $\nu_{iT'}$ & 0.266 & 0.270 & 0.199 & 0.347 & 1\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/number_parameters_population.tex <==

\begin{tabular}[b]{lrrrrr}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
$\mu^{\nu'}$ & -1.739 & -1.739 & -1.832 & -1.645 & 1.00\\
$\mu^{\mu^{^{\hat{r}'}}}$ & -0.822 & -0.817 & -0.962 & -0.695 & 1.00\\
$\mu^{\sigma^{^{\hat{r}'}}}$ & -0.269 & -0.260 & -0.583 & 0.021 & 1.03\\
$\mu_{T}^{\nu'} - \mu_{B}^{\nu'}$ & 0.348 & 0.349 & 0.200 & 0.484 & 1.00\\
$\sigma^{\nu'}$ & 0.269 & 0.268 & 0.218 & 0.321 & 1.00\\
\addlinespace
$\sigma^{\sigma^{^{\hat{r}'}}}$ & 0.045 & 0.040 & 0.005 & 0.094 & 1.03\\
$\sigma^{\mu^{^{\hat{r}'}}}$ & 0.350 & 0.304 & 0.044 & 0.776 & 1.02\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/number_parameters_transformed.tex <==

\begin{tabular}[b]{lllllll}
\toprule
  & mean & median & sd & hdi 2.5\% & hdi 97.5\% & $\hat{R}$\\
\midrule
\textit{Base Parameters:} &  &  &  &  &  & \\
Prior Std. Outcomes $\sigma^{\hat{r}'}$ & 0.774 & 0.772 & 0.118 & 0.544 & 1.005 & 1.03\\
Prior Mean Outcomes $\mu^{\hat{r}'}$ & 0.483 & 0.466 & 0.11 & 0.393 & 0.603 & 1.01\\
\addlinespace
\textit{Group Specific:} &  &  &  &  &  & \\
Noise Baseline $\nu'_{B}$ & 0.182 & 0.182 & 0.009 & 0.165 & 0.2 & 1\\
Noise Treatment $\nu'_{T}$ & 0.258 & 0.258 & 0.013 & 0.233 & 0.283 & 1\\
Weight on Numbers Baseline $\alpha'_B$ & 0.944 & 0.947 & 0.017 & 0.909 & 0.973 & 1.03\\
Weight on Numbers Treatment $\alpha'_T$ & 0.894 & 0.899 & 0.032 & 0.83 & 0.948 & 1.03\\
Prior Treshold Baseline $\delta'_B$ & 1.043 & 1.042 & 0.016 & 1.013 & 1.078 & 1.03\\
Prior Treshold Treatment $\delta'_T$ & 1.084 & 1.081 & 0.032 & 1.023 & 1.15 & 1.02\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/population_parameters.tex <==

\begin{tabular}[b]{lrrrrr}
\toprule
  & mean & sd & hdi 3\% & hdi 97\% & $\hat{R}$\\
\midrule
Mean $\nu$ Baseline $\mu_{B}^{\nu}$ & -1.554 & 0.049 & -1.645 & -1.460 & 1\\
Mean $\nu$ Treatment $\mu_{T}^{\nu}$ & -1.351 & 0.054 & -1.452 & -1.247 & 1\\
Diff. means $\nu$ $\mu_{T}^{\nu} - \mu_{B}^{\nu}$ & 0.203 & 0.073 & 0.060 & 0.334 & 1\\
Std. $\nu$ Baseline $\sigma_{B}^{\nu}$ & 0.543 & 0.041 & 0.469 & 0.622 & 1\\
Std. $\nu$ Treatment $\sigma_{T}^{\nu}$ & 0.604 & 0.047 & 0.515 & 0.690 & 1\\
\addlinespace
Mean $\frac{\beta}{1 - \beta}$ $\mu^{\frac{\beta}{1 - \beta}}$ & -0.770 & 0.035 & -0.837 & -0.706 & 1\\
Std. $\sigma^{\frac{\beta}{1 - \beta}}$ & 0.454 & 0.031 & 0.396 & 0.513 & 1\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/population_parameters_arithmetics.tex <==

\begin{tabular}[b]{lrrrrr}
\toprule
  & mean & sd & hdi 3\% & hdi 97\% & $\hat{R}$\\
\midrule
Mean $\nu$ Baseline $\mu_{B}^{\nu'}$ & -1.791 & 0.052 & -1.890 & -1.693 & 1\\
Mean $\nu$ Treatment $\mu_{T}^{\nu'}$ & -1.387 & 0.036 & -1.454 & -1.320 & 1\\
Diff. means $\nu$ $\mu_{T}^{\nu'} - \mu_{B}^{\nu'}$ & 0.404 & 0.063 & 0.290 & 0.525 & 1\\
Std. $\nu$ Baseline $\sigma_{B}^{\nu'}$ & 0.619 & 0.042 & 0.542 & 0.698 & 1\\
Std. $\nu$ Treatment $\sigma_{T}^{\nu'}$ & 0.403 & 0.029 & 0.349 & 0.459 & 1\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/population_parameters_prior.tex <==

\begin{tabular}[b]{lrrrr}
\toprule
  & mean & sd & hdi 3\% & hdi 97\%\\
\midrule
Mean $\nu$ Baseline $\mu_{B}^{\nu}$ & 0.090 & 1.042 & -1.673 & 2.255\\
Mean $\nu$ Treatment $\mu_{T}^{\nu}$ & 0.004 & 0.970 & -1.808 & 1.799\\
Diff. means $\nu$ $\mu_{T}^{\nu} - \mu_{B}^{\nu}$ & -0.087 & 1.428 & -2.382 & 2.830\\
Std. $\nu$ Baseline $\sigma_{B}^{\nu}$ & 0.790 & 0.600 & 0.002 & 1.869\\
Std. $\nu$ Treatment $\sigma_{T}^{\nu}$ & 0.797 & 0.618 & 0.003 & 1.972\\
\addlinespace
Mean $\frac{\beta}{1 - \beta}$ $\mu_{\frac{\beta}{1 - \beta}}$ & 0.039 & 0.981 & -1.742 & 1.909\\
Std. $\sigma_{\frac{\beta}{1 - \beta}}$ & 0.809 & 0.619 & 0.001 & 1.937\\
\bottomrule
\end{tabular}


==> graphs_export/structural_estimation/posterior_samples.tex <==
% Created by tikzDevice version 0.12.4 on 2023-12-21 09:26:09
% !TEX encoding = UTF-8 Unicode


==> graphs_export_restricted/structural_estimation/combined_parameters_prior.tex <==

\begin{tabular}[b]{lllll}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\%\\
\midrule
\textit{Individual Parameters (avg.):} &  &  &  & \\
Altr. Preference $\beta_i$ & 0.386 & 0.38 & 0.172 & 0.61\\
Noise $\nu_{\frac{\text{self}}{\text{other}},i}$ & 0.694 & 0.594 & 0.12 & 1.482\\
Noise $\nu_{\frac{\beta}{1- \beta},i}$ & 0.691 & 0.596 & 0.128 & 1.455\\
Prior Mean Outcomes $\mu^{\hat{r}}_i$ & 0.697 & 0.609 & 0.135 & 1.449\\
\addlinespace
\textit{Additional Parameter Information (avg.):} &  &  &  & \\
$\mu^{\nu_{\frac{\beta}{1-\beta}}}_B - \mu^{\nu_{\frac{\beta}{1-\beta}}}_T$ & 0.001 & 0.003 & -0.507 & 0.473\\
$\mu^{\nu_{\frac{\text{self}}{\text{other}}}}_B - \mu^{\nu_{\frac{\text{self}}{\text{other}}}}_T$ & -0.007 & -0.005 & -0.477 & 0.429\\
\bottomrule
\end{tabular}


==> graphs_export_restricted/structural_estimation/correlation_estimates_behavior.tex <==
[H]
\centering
\caption{Correlation Parameters Behavior \label{tab:params_correlations}}
\centering
\fontsize{10}{12}\selectfont
\begin{tabular}[b]{>{\raggedright\arraybackslash}p{4cm}>{\raggedright\arraybackslash}p{3cm}>{\raggedright\arraybackslash}p{3cm}l}
\toprule
  & Noise Altr. Preference $\nu_{\frac{\beta}{1-\beta}}$ & Noise Monetary Payments $\nu_{\frac{self}{other}}$ & Altr. Preference $\beta$\\
\midrule
\textit{Cognition-related:} &  &  & \\
No. Correct CRT & -0.327*** & -0.274*** & 0.126*\\
Berlin Numeracy Test & -0.247*** & -0.276*** & 0.173**\\
'I am good at math' & -0.197*** & -0.149** & 0.059\\
Avg. Need for Cognition & -0.150** & -0.163** & 0.125*\\
\addlinespace
Avg. Deliberation & 0.098 & 0.150** & -0.142*\\
Avg. Intuition & 0.066 & 0.119* & -0.097\\
 &  &  & \\
\textit{Altruism-related:} &  &  & \\
Dictator Game Other & -0.120* & -0.357*** & 0.495***\\
\addlinespace
GPS Donation & 0.063 & -0.049 & 0.146*\\
GPS Value Gift & -0.048 & -0.107 & 0.137*\\
MINT & 0.010 & 0.005 & 0.012\\
\bottomrule
\end{tabular}



==> graphs_export_restricted/structural_estimation/main_parameters_info_prior.tex <==

\begin{tabular}[b]{lrrrr}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\%\\
\midrule
$\mu^{\nu_{\frac{\beta}{1-\beta}}}_B - \mu^{\nu_{\frac{\beta}{1-\beta}}}_T$ & 0.001 & 0.003 & -0.507 & 0.473\\
$\mu^{\nu_{\frac{\text{self}}{\text{other}}}}_B - \mu^{\nu_{\frac{\text{self}}{\text{other}}}}_T$ & -0.007 & -0.005 & -0.477 & 0.429\\
\bottomrule
\end{tabular}


==> graphs_export_restricted/structural_estimation/main_parameters_prior.tex <==

\begin{tabular}[b]{lrrrr}
\toprule
  & mean & median & hdi 2.5\% & hdi 97.5\%\\
\midrule
Altr. Preference $\beta_i$ & 0.386 & 0.380 & 0.172 & 0.610\\
Noise $\nu_{\frac{\text{self}}{\text{other}},i}$ & 0.694 & 0.594 & 0.120 & 1.482\\
Noise $\nu_{\frac{\beta}{1- \beta},i}$ & 0.691 & 0.596 & 0.128 & 1.455\\
Prior Mean Outcomes $\mu^{\hat{r}}_i$ & 0.697 & 0.609 & 0.135 & 1.449\\
\bottomrule
\end{tabular}


==> input/outline_session.tex <==
% Define box styles
\tikzstyle{box} = [rectangle, draw, text centered, rounded corners, minimum height=1cm, minimum width = 16cm, line width=0.5mm]
\tikzstyle{box_title} = [rectangle, draw=white, text centered, minimum width = 3cm]
\tikzstyle{line} = [draw, -latex']

\tikzstyle{box_a} = [rectangle, draw, text centered, rounded corners, minimum height=1cm, minimum width = 7cm, line width=0.5mm]
\tikzstyle{bigbox_a} = [draw=black, loosely dotted, line width=0.75mm, rounded corners, rectangle, minimum height=7cm, minimum width = 17.5cm]
\tikzstyle{bigbox_b} = [draw=black, loosely dotted, line width=0.75mm, rounded corners, rectangle, minimum height=8.2cm, minimum width = 17.5cm]



\begin{tikzpicture}[auto, node distance=25mm, scale=0.7, every node/.style={scale=1},
    mylabel/.style={label={above left:{#1}}}]

    % Place nodes

    \node [box, align=center, text width=16cm] (stage1) {\textbf{Part 1: Altruistic Choices} \\
        %\vspace{-0.25cm}
        \begin{itemize}
            \setlength{\itemsep}{2pt}
            \setlength{\parskip}{0pt}
            \setlength{\parsep}{0pt}
            \item Decide between taking payment $\text{self}$ or giving $\text{other}$. 240 total trials with intermediate breaks possible. 
            \item One decision randomly implemented at the end of the experimental session.
        \end{itemize}
     };

    \node [box, align=center, text width=16cm, below=10pt of stage1] (stage2) {\textbf{Part 2: Number Comparison} \\
        %\vspace{-0.25cm}
        \begin{itemize}
            \setlength{\itemsep}{2pt}
            \setlength{\parskip}{0pt}
            \setlength{\parsep}{0pt}
            \item Judge which of two numbers $\text{A}$ (previously $\text{self}$) or $\text{B}$ (previously $\text{other}$) $\times \sfrac{1}{2}$ is larger. 200 trials total.
         	\item Final payment = $10$ \EUR $\times$ avg. correct - avg. time in seconds.
        \end{itemize}
    };

    \node [box, align=center, text width=16cm, below=10pt of stage2] (stage3) {\textbf{Part 3: Additional Data} \\
        %\vspace{-0.25cm}
        \begin{itemize}
            \setlength{\itemsep}{2pt}
            \setlength{\parskip}{0pt}
            \setlength{\parsep}{0pt}
            \item Dictator Game 10 featuring \EUR, implemented with 1\% probability.
            \item Social and Private Norm Elicitation for Altruistic Choices, both for Baseline and Treatment variant; "Excuses" Survey
            \item Cognitive Reflection Task, Berlin Numeracy Test
            \item Surveys (Preferences for Deliberation and Intuition, GPS Altruism, Need for Cognition, Machiavellianism)
            \item Demographics
        \end{itemize}
    };





\end{tikzpicture}

